Tackling Combinatorial Distribution Shift: A Matrix Completion Perspective

Obtaining rigorous statistical guarantees for generalization under distribution shift remains an open and active research area. We study a setting we call combinatorial distribution shift, where (a) under the test- and training-distributions, the labels $z$ are determined by pairs of features $(x,y)$, (b) the training distribution has coverage of certain marginal distributions over $x$ and $y$ separately, but (c) the test distribution involves examples from a product distribution over $(x,y)$ that is {not} covered by the training distribution. Focusing on the special case where the labels are given by bilinear embeddings into a Hilbert space $H$: $\mathbb{E}[z \mid x,y ]=\langle f_{\star}(x),g_{\star}(y)\rangle_{{H}}$, we aim to extrapolate to a test distribution domain that is $not$ covered in training, i.e., achieving bilinear combinatorial extrapolation. Our setting generalizes a special case of matrix completion from missing-not-at-random data, for which all existing results require the ground-truth matrices to be either exactly low-rank, or to exhibit very sharp spectral cutoffs. In this work, we develop a series of theoretical results that enable bilinear combinatorial extrapolation under gradual spectral decay as observed in typical high-dimensional data, including novel algorithms, generalization guarantees, and linear-algebraic results. A key tool is a novel perturbation bound for the rank-$k$ singular value decomposition approximations between two matrices that depends on the relative spectral gap rather than the absolute spectral gap, a result that may be of broader independent interest.

==> body/Formulation.tex <==
\section{Problem Formulation}\label{sec:formulation} 


==> body/body.tex <==
%!TEX root = ../colt_main.tex

\section{Introduction}
For the sake of concreteness, we focus on the problem of separating marbles of different colors $k \in [K]$ into piles of discrete colored marble. The goals of this investigation are as follows:
\begin{enumerate}
	\item Separating marbles into piles is a dextrous manipulation task which is straightforward for humans, but remains challenging for robots. 
	\item Human beings have a capacity to execute ``high level'' plans whereby they group multiple marbles together, to move them as a unit. This requires representation of the marbles as a single, cohesive unit, which is not only \emph{task specific} (one could imagine, for example, separating colors $\{1,2,\dots,K/2\}$ from $\{K/2 + 1,\dots,K\}$), but also \emph{policy specific}, in that the group manipulated together depends on the humans action. 
	\item We consider a strategy whereby a high-level planner reasons about which groups of marbles to manipulate, but a low-level planner considers how to maintain the integrity of these groups as a cohesive unit. The upshot is that the high-level planner need not worry about planning through a sophisticated particle simulation of all marbles. Moreover, the low-level planner may be sub-optimal, and needs only to enforce cohesiveness. 
	\item What may facillate such a simple low-level planner are the following observations: (a) it is perhaps possible to focus only on the perimeter of the marbles in the clump, and ensure that no marble leave said perimeter (b) of course, movement of the clump will be lost some internal kinetic energy of the marbles themselves. One may hope that this difference in dynamics between a single rigid object and multiple can be adressed by stabilizing at a high level (c) one may hope that only coarse dynamic information need be collected to prevent marbles from behaving erratically. 
	\item Ideally, we do not want to rely on object identity (tracking every single marble). Humans need not do this. 
	\item We wish to avoid a trivial algorithm which moves each marble one at a time.
\end{enumerate}

\newcommand{\lab}{\mathsf{lab}}
\newcommand{\matq}{\mathbf{q}}
\newcommand{\tfin}{t_{\mathrm{f}}}
\section{Problem statement}
We consider a finite set of marbles $z \in \cZ$. To each marble, we associate a state, $\matx_z(t) \in \R^d$, which may include position information, velocity, and rotational dynamics. The center of each marble is denote $\matq_z(t) \in \R^3$, which we assume comprises the first three coordinates of $\matx_z$. 

We also associated its color, or more general, \emph{label,} $\lab_z \in [K]$ for $K \in \N$ labels. We are given a set of $K$ disjoint\footnote{we assume disjointness for now for simplicity} convex regions $\cC_1,\dots,\cC_K$, and the goal is ensure that, at some $\tfin$, one has
\begin{align*}
\{\matq_z(\tfin) : \label_z = k, z \in \cZ\} \subset \cC_k, \quad \forall k \in [K].
\end{align*}
One may be able to formulate a planning objective which attempts to minimize $\tfin$, and enforces other smoothness constraints. 

Of particular interest is the setting where $K = 2$ (e.g. red and blue marbles), and the marbles are arranged in a circle with red and blue marbles on either side, but touching down the middle. 

We assume access to cameras, which, for every $z \in \cZ$, return \emph{exact} measurements of $\matq_z(t)$, as well as \emph{perfectly} identify the label $\label_z$. The camera need not be able to distinguish the particular index of the marble (e.g. if $z,z' \in \cZ$ have $\lab_{z} = \lab_{z'}$, the two may be indistinguishable.) \mscomment{How to formalize}

\newcommand{\planner}{\mathsf{P}}
\newcommand{\pprop}{\planner_{\mathtt{prop}}}
\newcommand{\phigh}{\planner_{\mathtt{hi}}}
\newcommand{\plow}{\planner_{\mathtt{low}}}

\section{A candidate representation}
We consider the following candidate for representation:
\begin{enumerate}
	\item A high level planner identifies clumps of marbles which are adjacent which are capable of being moved. We call this the proposal planner $\pprop$.
	\item A second high level planner $\phigh$ plans a movement for these marbles as if they are an \emph{fixed clump}.
	\item A low level planner $\plow$ ensures that the marbles behave as a continuous clump.
\end{enumerate}
Importantly, $\pprop$ and $\phigh$ need only take into account geometric information. On the other hand, $\plow$ ensures may rely on particle simulation, but perhaps can use precomputed, or offline policies. The 

The key idea is that the high level planner \emph{determines} the representation, and the low level planner \emph{enforces it}. We can even have the high level planner include the target representation a part of the plan. 

The low level planner is pure stability, so does not require ``exploration'' in a traditional sense? Perhaps it can be trained from behavioral cloning where we tell the robot to move a clump, and the loss suffered is the deviation from the clump \mscomment{formalize this}. This planner should learn things like, applying too much force squeezes the marbles together and can make them shoot off in various directions. 

\subsection{Observations}
In some sense, we do not wish to model all marbles at once, even in the low level planner. I propose a different criterion for state representation called \mscomment{some name}. Under this criterion, the states represented are the particles that seem to be going awry (for example, marbles on the perimeter that are going too fast). Need to think more. 

==> body/concrete_formulation.tex <==
%!TEX root = ../main.tex

\section{Concrete Formulation} 
We consider the following model for representing the transfer:\kz{a bit confused about the following formulation's notation: the same $\pi$ on both sides in the second equation? are we solving a fixed-point equation?}
\begin{align}
\psi(g,g') &= f_\phi(g' - g) \\
 \pi(x,g') &= h_{\psi(g,g')}(x,\pi(x,g)).
\end{align}
For simplicity, we make the following assumptions: 
\begin{enumerate}
	\item The spline $h_{\psi}(x,a)$ takes the form
	\begin{align*}
	h_{\psi}(x,a) = \Phi(x,a) \psi, 
	\end{align*}
	where $\Phi(x,a)$ is unlearned. 
\end{enumerate}

\subsection{Training with a generative model}
\newcommand{\data}{\hat{\cD}}
\newcommand{\distr}{\cD}
\newcommand{\Dtrain}{\cD_{\mathrm{train}}}

\newcommand{\datatrainnew}{\data_{\mathrm{train}}'}
\newcommand{\datatrainold}{\data_{\mathrm{train}}}
\newcommand{\distrainnew}{\distr_{\mathrm{train}}'}
\newcommand{\distrainold}{\distr_{\mathrm{train}}}
\newcommand{\kNN}{k\text{-NN}}
\newcommand{\phitrain}{\hat{\phi}}
\newcommand{\Ltesthat}{\hat{\cL}_{\mathrm{test}}}
\newcommand{\Ltest}{\cL_{\mathrm{test}}}

\newcommand{\testsub}{\mathsf{ts}}
\newcommand{\gtest}{g^{\testsub}}
\newcommand{\stest}{s^{\testsub}}
\newcommand{\atest}{a^{\testsub}}
\newcommand{\Ntest}{N_{\testsub}}
\newcommand{\gtesti}{g^{\testsub}_i}
\newcommand{\stesti}{s^{\testsub}_i}
\newcommand{\atesti}{a^{\testsub}_i}
\newcommand{\distest}{\distr_{\testsub}}
\newcommand{\xtest}{x^{\testsub}}
\newcommand{\xtesti}{x^{\testsub}_i}


\newcommand{\Dtest}{\cD_{\mathrm{test}}}

We assume that we have the following data sets\kz{how shall we design $\distrainnew$ and $\distrainold$ such that the difference distribution, i.e., the distribution of $g'_{i}-g_{i}$, is ``representative'' enough?}
\begin{align}
g'_{1},\dots,g'_{N'} &\iidsim \distrainnew\\
(g_1,s_1,a_1),\dots (g_N,s_N,a_N) &\sim \distrainold
\end{align}
We introduce a weighting function $\omega(g',g;g_{1:N})$ such that, 
\begin{align}
\forall g' \in \cG, \quad \sum_{i=1}^n\omega(g',g_i;g_{1:N}) = 1.
\end{align}
For example, letting $\kNN(g';g_{1:N})$ denote the set of $k$-Nearest Neighbors of $g'$ in $\{g_1,\dots,g_N\}$ (ties broken arbitrarily), then we can use the $k$-NN averaging to be
\begin{align*}
\omega(g',g_i;g_{1:N}) := \begin{cases} \frac{1}{k} & g_i \in \kNN(g';g_{1:N})\\
0 & \text{otherwise}
\end{cases}
\end{align*}
To train, we propose the following \kz{so not a fixed point, but getting $\pi$ from previous training.}
\begin{align*}
\phitrain \in \argmin_{\phi} \sum_{i=1}^{N'} \left(\sum_{j=1}^N \omega(g_i',g_j;g_{1:N})\|\Phi(s_j,a_j)f_{\phi}(g'_i-g_j)-\pi(x_j,g')\|_2^2\right)
\end{align*}
Then, to test, we draw\kz{is the difference between the loss above and below on purpose?}
\begin{align*}
(\gtesti,\xtesti,\atesti) \iidsim \distest
\end{align*}
\begin{align*}
\Ltesthat(\phitrain) := \frac{1}{\Ntest}\sum_{i =1}^{\Ntest} \left\|\left(\sum_{j=1}^N \omega(\gtesti,g_j;g_{1:N})\Phi(\xtesti,\pi(\xtesti,g_j))f_{\phi}(\gtesti-g_j)\right) - \atesti\right\|_2^2
\end{align*}

\subsection{Out of distribution: globally linear weights}
\newcommand{\Ltrain}{\cL_{\mathrm{train}}}
\newcommand{\phist}{\phi_{\star}}
\newcommand{\Dgen}{\cD_{\mathrm{gen}}}
So, lets say $\omega(\gtesti,g_j;g_{1:N}) = 1/N$, so that there is no localization of the weight. Introduce the population losses
\begin{align*}
\Ltrain(\phi) &:= \Exp_{g' \sim \distrainnew}\Exp_{(x,a,g)\sim \distrainold}\|\Phi(x,a)f_{\phi}(g' - g)-\pi(x,g')\|_2^2\\
\Ltest(\phi) &= \Exp_{(\gtest,\xtest,\atest) \sim \Dtest}\|\Exp_{g\sim \Dgen(\gtest)}\Phi(\xtest,\pi(\xtest,g))f_{\phi}(\gtest - g) -\atest\|_2^2
\end{align*}

\newcommand{\distrchtrain}{\distr_{\mathrm{\Delta},\mathrm{train}}}
\newcommand{\distrchtest}{\distr_{\mathrm{\Delta},\mathrm{test}}}

\newcommand{\delg}{\updelta  g}
\newcommand{\Lamtrain}{\Lambda_{\mathrm{train}}}
\newcommand{\Lamtest}{\Lambda_{\mathrm{test}}}

\begin{lemma}\label{lem:del_g_loss} Introduce $\distrchtrain$ as the law of $g'-g$ where $g,g' \iidsim \Dtrain$ in the training data, and $\distrchtest$ as the law of $\gtest - g$, where $\gtest \sim \Dtest$ and $g \sim \Dgen$ are independent.  Further, define
\begin{align*}
\Lamtrain(\delg) &:= \Exp_{(x,a) \mid \delg \sim \distrchtrain}\Phi(x,a)^\top\Phi(x,a)\\
\Lamtest(\delg) &:= \Exp_{(g,\xtest)\sim \Dgen \times \Dtest \mid  \delg \sim \distrchtrain}\Phi(\xtest,\pi(\xtest,g))^\top \Phi(\xtest,\pi(\xtest,g))
\end{align*}
Then, assuming realizability, 
\begin{align*}
\Ltrain(\phi) &= \Exp_{\delg \sim \distrchtrain}\|f_{\phi}(\delg)-f_{\phi_{\star}}(\delg )\|_{\Lamtrain(\delg)}^2\\
\Ltest(\phi) &=  \Exp_{\delg \sim \distrchtest}\|f_{\phi}(\delg)-f_{\phi_{\star}}(\delg )\|_{\Lamtest(\delg)}^2
\end{align*}
\end{lemma}
\begin{proof}[Proof of \Cref{lem:del_g_loss}]
Write
\begin{align*}
\Ltrain(\phi) &= \Exp_{g' \sim \distrainnew}\Exp_{(x,a,g)\sim \distrainold  }\|\Phi(x,a)f_{\phi}(\del g)-\pi(x,\delg + g)\|_2^2 \\
&= \Exp_{\delg \sim \distrchtrain}\Exp_{(x,a,g)\sim \distrainold \mid \delg  \sim \distrchtrain}\|\Phi(x,a)f_{\phi}(\del g)-\pi(x,\delg + g)\|_2^2.
\end{align*}
Assuming realizability, 
\begin{align*}
\Ltrain(\phi) &= \Exp_{g' \sim \distrainnew}\Exp_{(x,a,g)\sim \distrainold  }\|\Phi(x,a)(f_{\phi}(g' - g)-f_{\phi_{\star}}(g - g'))\|_2^2 \\
&= \Exp_{\delg \sim \distrchtrain}\Exp_{(x,a,g)\sim \distrainold  \mid \distrchtrain}\|\Phi(x,a)(f_{\phi}(\delg)-f_{\phi_{\star}}(\delg ))\|_2^2 \\
&= \Exp_{\delg \sim \distrchtrain}\Exp_{(x,a) \mid \delg \sim \distrchtrain}\|(f_{\phi}(\delg)-f_{\phi_{\star}}(\delg ))\|_{\Phi(x,a)^\top \Phi(x,a)} \\
&= \Exp_{\delg \sim \distrchtrain}\|f_{\phi}(\delg)-f_{\phi_{\star}}(\delg )\|_{\Lamtrain(\delg)}^2
\end{align*}

Similary, with ``infinite data'' (maybe re-sampling $(x,a,g)$ to avoid correlation), 
\begin{align*}
\Ltest(\phitrain) 
&= \Exp_{(\gtest,\xtest,\atest) \sim \Dgen}\|\Exp_{g\sim \Dtrain}\Phi(\xtest,\pi(\xtest,g))f_{\phitrain}(\gtest - g) -\atest\|_2^2\\
&= \Exp_{(\gtest,\xtest,\atest) \sim \Dgen}\|\Exp_{g\sim \Dtrain}\Phi(\xtest,\pi(\xtest,g))[f_{\phitrain}(\gtest - g) -f_{\star}(\gtest - g)\|_2^2\\
&= \Exp_{\delg \sim \distrchtest}\|\Exp_{(g,\xtest)\sim \Dtrain \times \Dgen \mid  \delg \sim \distrchtrain}\Phi(\xtest,\pi(\xtest,g))[f_{\phitrain}(\delg) -f_{\star}(\delg)\|_2^2\\
&= \Exp_{\delg \sim \distrchtest}\|f_{\phitrain}(\delg) -f_{\star}(\delg)\|_{\Lamtest(\delg)}^2
\end{align*}
\end{proof}


\newcommand{\rDel}{\mathsf{r}_{\Delta}}
\newcommand{\rLam}{\mathsf{r}_{\Lambda}}
\newcommand{\remai}{\mathsf{rem}}

\begin{lemma}
Suppose that $\sup_{\phi,\delg}\|f_{\phi}(\delg)\|\le B$, and define
\begin{align*}
\rLam(\delg;\lambda) &:= \|(\Lamtrain(\delg) + \lambda I )^{-\frac{1}{2}}\Lamtest(\delg)^{1/2}\|_{\op}^2\\
\rDel(\delg) &:= \frac{\rmd \distrchtest(\delg)}{\rmd \distrchtrain(\delg)}\\
\remai(\lambda) &:= \lambda B^2 \Exp_{\delg \sim \distrchtest}\left[\rLam(\delg;\lambda)\right].
\end{align*}
 Then, 
\begin{align*}
\Ltest(\phi) \le \inf_{\lambda \ge 0} \left(\min \left\{\begin{matrix} \Ltrain(\phi) \cdot \sup_{\delg}\rLam(\delg;\lambda)\rDel(\delg)\vspace{.2em}\\\sqrt{\Ltrain(\phi)}\cdot \sqrt{\Exp_{\delg \sim \distrchtrain}\rLam(\delg;\lambda)^2\rDel(\delg)^2}\end{matrix}\right\} + \remai(\lambda)\right) 
\end{align*}
\end{lemma}
\begin{proof}
\begin{align*}
\Ltest(\phi) &=  \Exp_{\delg \sim \distrchtest}\left[\|f_{\phi}(\delg)-f_{\phi_{\star}}(\delg )\|_{\Lamtest(\delg)}^2\right]\\
&\le  \Exp_{\delg \sim \distrchtest}\left[\|f_{\phi}(\delg)-f_{\phi_{\star}}(\delg )\|_{\Lamtrain(\delg) + \lambda I }^2 \cdot \sup_{v \ne 0}\frac{\|v\|_{\Lamtest(\delg)}}{\|v\|_{\Lamtrain(\delg) + \lambda I }}\right]\\
&\le  \Exp_{\delg \sim \distrchtest}\left[\|f_{\phi}(\delg)-f_{\phi_{\star}}(\delg )\|_{\Lamtrain(\delg) + \lambda}^2 \|\Lamtrain(\delg) + \lambda I )^{-\frac{1}{2}}\Lamtest(\delg)\Lamtrain(\delg) + \lambda I )^{-\frac{1}{2}}\|_{\op}\right]\\
&:= \Exp_{\delg \sim \distrchtest}\left[\|f_{\phi}(\delg)-f_{\phi_{\star}}(\delg )\|_{\Lamtrain(\delg) + \lambda}^2 \rLam(\delg;\lambda)\right]\\
&= \Exp_{\delg \sim \distrchtest}\left[\|f_{\phi}(\delg)-f_{\phi_{\star}}(\delg )\|_{\Lamtrain(\delg)}^2 \rLam(\delg;\lambda)\right] + \lambda B^2 \Exp_{\delg \sim \distrchtest}\left[\rLam(\delg;\lambda)\right]\\
&\le \Exp_{\delg \sim \distrchtrain}\left[\|f_{\phi}(\delg)-f_{\phi_{\star}}(\delg )\|_{\Lamtrain(\delg)}^2 \rLam(\delg;\lambda)\left(\frac{\rmd \distrchtest(\delg)}{\rmd \distrchtrain(\delg)} \right)\right] + \lambda B^2 \Exp_{\delg \sim \distrchtest}\left[\rLam(\delg;\lambda)\right]\\
&= \Exp_{\delg \sim \distrchtrain}\left[\|f_{\phi}(\delg)-f_{\phi_{\star}}(\delg )\|_{\Lamtrain(\delg)}^2 \rLam(\delg;\lambda)\rDel(\delg)\right] + \lambda B^2 \Exp_{\delg \sim \distrchtest}\left[\rLam(\delg;\lambda)\right]\\
\end{align*}
We now derive two upper bounds. First,
\begin{align*}
&\Exp_{\delg \sim \distrchtrain}\left[\|f_{\phi}(\delg)-f_{\phi_{\star}}(\delg )\|_{\Lamtrain(\delg)}^2 \rLam(\delg;\lambda)\rDel(\delg)\right] \\
&\quad\le \left(\sup_{\delg}\rLam(\delg;\lambda)\rDel(\delg)\right)\Exp_{\delg \sim \distrchtrain}\|f_{\phi}(\delg)-f_{\phi_{\star}}(\delg )\|_{\Lamtrain(\delg)}^2 \\
&\qquad= \left(\sup_{\delg}\rLam(\delg;\lambda)\rDel(\delg)\right)\Ltrain(\phi).
\end{align*}
On the other hand, by Cauchy-Schwartz,
\begin{align*}
&\Exp_{\delg \sim \distrchtrain}\left[\|f_{\phi}(\delg)-f_{\phi_{\star}}(\delg )\|_{\Lamtrain(\delg)}^2 \rLam(\delg;\lambda)\rDel(\delg)\right]\\
&\quad\le \sqrt{\Exp_{\delg\sim \distrchtrain}\rLam(\delg;\lambda)^2\rDel(\delg)^2}\sqrt{\Exp_{\delg \sim \distrchtrain}\|f_{\phi}(\delg)-f_{\phi_{\star}}(\delg )\|_{\Lamtrain(\delg)}^2} \\
&\quad\le \sqrt{\Exp_{\delg \sim \distrchtrain}\rLam(\delg;\lambda)^2\rDel(\delg)^2}\sqrt{\Ltrain(\phi)}.
\end{align*}
\end{proof}



\newcommand{\Dgoaltrain}{\cD_{\mathrm{goal,tr}}}
\newcommand{\Dgoaltest}{\cD_{\mathrm{goal,tst}}}
\newcommand{\Unif}{\mathrm{Unif}}
\newcommand{\ratioooddel}{r_{\mathrm{OOD},\Delta}}
\newcommand{\ratioood}{r_{\mathrm{OOD}}}


\subsection{Goal Space is a line}
Consider a goal space where $\Dtrain(\cG) = \Unif[\alpha_1,\alpha_2]$, and $\Dtest(\cG) = \Unif[\alpha_2,\alpha_3]$. Suppose $\Dgen = \Unif[\alpha_2 - \eta,\alpha_2]$. Then,
\begin{align*}
\end{align*}




\section{Algorithmic Choices}

\subsection{Choosing $\Dgen$}
How do we choose comparison tasks? We can sample from nearest, neighbors, but this is bad:
\begin{lemma}\mscomment{TODO: Why is nearest neighbors bad? Poor SNR. Prove lower bond}
\end{lemma}


\subsection{Adversarial Training}

\begin{align*}
\bar{\ell}_t( f_{\phi}, \Lambda_{\varphi} ;\delg) = \|f_{\phi}(\delg) - f_{\phi_\star}(\delg)\|_{\Lambda_{\varphi}(\delg)}^2
\end{align*}
The min player plays $f_{\phi}$, the max player plays $z_{\varphi}$ where
\begin{align*}
\Exp_{\delg}\Exp_{(x,a)\sim z_{\varphi}(\delg)} \Phi(x,a)^\top \Phi(x,a) = \Lambda_{\varphi}(\delg).
\end{align*}


\section{The factorial generalization problem}
\newcommand{\Dtrainx}{\cD_{\cX,\mathrm{train}}}
\newcommand{\Dtrainz}{\cD_{\cZ,\mathrm{train}}}
\newcommand{\Dtestx}{\cD_{\cX,\mathrm{test}}}
\newcommand{\Dtestz}{\cD_{\cZ,\mathrm{test}}}
\newcommand{\kapx}{\kappa_{\cX}}
\newcommand{\kapz}{\kappa_{\cZ}}

Consider a joint distribution over environments contexts:
\begin{align*}
(x,z) \in \cX \times \cZ \sim \Dtrain,
\end{align*}
whose marginals are $\Dtrainz$ and $\Dtrainz$. We call $x$ the \emph{context}, and $z$ the \emph{environment}. Policies operate as $\pi: \cX \times \cZ \to \cA$ Here are some examples:
\begin{example}[Block Pushing]  The environments are a set of blocks $\cZ_0$ whose dimension are vectors $z \in \R^{d_z}$. The goal is to push the block to a set of some locations $\cP_0 \in \R^{2}$. Given some compact observation of the block (e.g. pose $y \in \R^{k}$), the context is $x = (p,y) \in \R^2 \times \R^k$ is the pair of goal location and observation. 
\end{example}

\begin{example}[Cup Manipulation] The environments are a set of cups $\cZ_0$ whose dimension are vectors $z \in \R^{d_z}$, the goal is a number of tasks parametrized abstractly by $x \in \cX$. We consider learning an open-loop policy, and without loss of generality, we wish to learn the policy at a fixed time step $t$. Hence, for each $t$, we consider $\pi(x,z;t)$ which is the open loop mapping taking cup $z$ and state $x$ to the output.
\end{example}

Our goal is to imitate a policy $\pi(z,x)$ on some other distribution
\begin{align*}
(x,z) \sim \Dtest,
\end{align*}
whose marginals are $\Dtestx$ and $\Dtestz$. We assume bound distributioned shift on the marginals:
\begin{align*}
\sup_{z}\frac{\rmd \Dtestz(z)}{\rmd \Dtrainz(z)} \le \kapz \quad \sup_{x}\frac{\rmd \Dtestx(x)}{\rmd \Dtrainx(x)}  \le \kapx.
\end{align*} 
Importantly, we \emph{do not} assume a bounded density ratio on the joint distributions, and in fact, we may have
\begin{align*}
\sup_{(x,z)} \frac{\rmd \Dtest(x,z)}{\rmd \Dtrain(x,z)} = \infty. 
\end{align*}

We consider the following class of models
\begin{align*}
\pihat_{\phi}(x,z') = h_{\psi}(\Phi(x,z')), \quad \psi = f_{\phi}(z' -z)
\end{align*}

\begin{example}[Block Pushing to End Regions] 
\end{example}

\subsection{Things}
In this paradigm, what can we control?
\begin{enumerate}
	\item 
\end{enumerate}

==> body/concrete_formulation_old.tex <==
%!TEX root = ../main.tex

\section{Concrete Formulation}
\newcommand{\matN}{\mathbf{N}}
\newcommand{\Fclass}{\mathscr{F}}
\newcommand{\distr}{\triangle}
\newcommand{\wst}{w^{\star}}
\subsection{Thin plane splines}
Abhishek is implenting these with thin-plate splines. We consider a target degree of smoothness $m$ satisfying $m > 2d$, and now that spline minimizers take the form \mscomment{remember a citation}
\begin{align*}
g(\matx) = \sum_{i=1}^n \beta_{i} \eta_{md}(\|\matx - \matx_i\|) + \sum_{j=1}^M \alpha_j \phi_j(\matx)
\end{align*}
where above $M = \binom{m+d-1}{d}$. If we collect $\phi_j$ into $\bPhi$, and $\alpha_j$ into $\balpha$, $\beta_i$ into $\bbeta$, and $\matN_{i,j} = (\eta_{md}(\|\matx_j - \matx_i\|))$, then 
\begin{align*}
g(\matx_i) = \matN \bbeta + \bPhi \balpha,
\end{align*}
We further require $\bPhi^\top \bbeta = 0$, leading to a regularized regression problem
\begin{align*}
\min_{\bbeta,\balpha} \|\maty -  (\matN \bbeta + \bPhi \balpha)\|_2^2 + \lambda \bbeta^\top \matN \bbeta: \bPhi^\top \bbeta = 0.
\end{align*}
\mscomment{How to make this function class work with the smoothing!? Opportunity for challenge :) }

\subsection{A simplification with a linear function class}
Let us put things in adams notation. We will let $h$ denote the spline, which for simplicity we write as linear in a basis. That is
\begin{align*}
h(a;\balpha) = \sum_{i=1}^k \alpha_i\cdot \phi_i(a).
\end{align*}

\paragraph{Option 1: Continuous, but Deterministic Actions}
With continuous but deterministic actions, we we consider $\cA \subset \R^{d_a}$, and consider a loss
\begin{align*}
\ell(a',a) := \|a' - a\|^2,
\end{align*}
or more generall a convex loss. We further have a class of functions $f \in \Fclass$ for which 
\begin{align*}
\Fclass: (g-g') \in \cG  - \cG \mapsto \balpha.
\end{align*}
In this case, if we set
\begin{align*}
\tilde{\ell}(\balpha,a,a') = \|h(a;\balpha) - a'\|^2,
\end{align*}
then 
\begin{align*}
\ell(h(a;f(g-g')), a')  = \tilde{\ell}(f(g-g'),a,a'). 
\end{align*}
Notice that since $\tilde{\ell}(\balpha,a,a')$ is convex in its first argument, the conditions of Adam's paper hold, and one can get bounded regret.

\paragraph{Option 2: Discrete, but Randomized Actions}
Here, we can use something like a logistic loss instead. The key property is that, for any $p \in \distr(\cA)$ and matrix $\bPhi$,
\begin{align*}
\balpha \mapsto \ell( \bPhi \balpha, p(\cdot)) \text{is convex and Lipschitz}.
\end{align*}


\subsection{}
\newcommand{\Dtrain}{\cD_{\mathrm{train}}}
\newcommand{\delg}{\updelta g}
\begin{align*}
\Exp_{g,g',s,a \sim \Dtrain}\| f_{\phi}(\delg) - f_{\star}(\delg) \|_{\Phi(s,a)^\top \Phi(s,a)}^2 = \Exp_{g,g' \sim \Dtrain}\| f_{\phi}(\delg) - f_{\star}(\delg) \|_{\Lambda_{g,g'} \sim \Dtrain}^2
\end{align*}

\subsection{Goal Selections}
\subsection{Immitation Learning}
\newcommand{\fhat}{\hat{f}}
\newcommand{\dist}{\mathsf{dist}}
\section{Adversarial Training}
Consider the previous section. We consider how to select a training of distribution of actions, given a certain direction $g-g' \in \cG- \cG$. 
\subsection{A linear game}
Suppose that I have a linear function $\fst(\matx) = \langle \wst, \matx \rangle$. Suppose that I want learn a linear $\fhat$ such that $\dist(\fst,f) := \sup_{\matx:\|\matx\|_2 \le 1} |\fst(\matx) - \fhat(\matx)| \le \epsilon$.

Consider a noiseless variant, with bandit feedback, where I query $\matx_t$, and receive $\maty_t - \fst(\matx_t)$. Then, clearly, I can learn $\fst$ with $T = d$ queries with, say, $(\matx_1,\dots,\matx_d) = (\mate_1,\dots,\mate_d)$, the cannonical basis vectors. 
Consider the following game:
\begin{enumerate}
	\item At each time $t$, I play an $\fhat_t$. 
	\item Then, I sample a $\matx_t$.
\end{enumerate}
Suppose that both sequences satisfy an \emph{low regret guarantee} on
\begin{align*}
R_{1,T} &:= \sum_{t=1}^T (\fhat_t(\matx_t) - \maty_t)^2 - \inf_{f \in \Fclass}\sum_{t=1}^T (f(\matx_t) - \maty_t)^2 \\
R_{2,T} &:=  \sup_{\matx \in \cX}\sum_{t=1}^T (\fhat_t(\matx) - \maty_t)^2 - \sum_{t=1}^T (\fhat_t(\matx_t) - \maty_t)^2
\end{align*}
Can we argue that such a learner can produce an $f$ such that
\begin{align*}
\sup_{\matx}\left( \Exp[(\fhat(\matx) - \maty_t)^2 \mid \matx] - \inf_{f \in \Fclass} \Exp[f(\matx) - \maty_t)^2 \mid \matx]\right) \le \text{small}?
\end{align*}
Linear case
\begin{align*}
V_T(\what_{1:T},\matx_{1:T}) &= \sum_{t=1}^T \langle \matx_t, \what_t -  \wst\rangle^2 \\
&= \sum_{t=1}^T \|\what_t -  \wst\|_{\matX_t}^2, \quad \matX_t = \matx_t \matx_t^\top
\end{align*}
So then 
\begin{align*}
V_T(\bar{w},\matx_{1:T}) &= \sum_{t=1}^T \|\bar{\matw} -  \wst\|_{\matX_t}^2 \\
&\le V_T(\what_{1:T},\matx_{1:T}) \tag{Jensen's inequality}\\
&\le V_T(\wst,\matx_{1:T}) +  R_{1,T} \tag{Regret Def}
\end{align*}

==> body/illustrations.tex <==
%!TEX root = ../main.tex


\section{What kind of settings?}


\subsection{What problems is this?}
We want to apply this to a broader set of control problems/prediction problems than just simply low-rank problems. For example, we might imagine that the embeddings  look like 
\begin{align*}
\fst(x) = \sum_{n \ge 0}\alpha_n \cos(nx + \omega_{n})\\
\gst(y) = \sum_{n \ge 0} \beta_n \cos(ny + \nu_{n}),
\end{align*}
where $\alpha_n,\beta_n$ have gradual decay. We also want to remove the condition that you are uniformly sampling blocks from a matrix, but instead can do ERM on some training distribution. 

\subsection{Questions}
\begin{itemize}
	\item Is this signifcant? Has this been done?
	\item Are there related work in the literature?
	\item Are there other problems for us to consider?
\end{itemize}

\subsection{Statement}


\begin{align*}
 %\Risk(\ffin,\gfin;\Dtest)  &\le c\left(\ErrTermPred + \frac{\poly(\rred)\ErrTermOver}{\sigma_{\rred}(\Sigst)^2} + \frac{\tailsf_2(\rred)^2}{\sigma_{\rred}(\Sigst)^2} +  \tailsf_1(\rred)^2 \right).
 %c_3 \po \left(\ErrTerm + (r+\kpick^4)\ErrTerm + \frac{s^6 }{\sighat_r^2}\ErrTerm^2 + \frac{\left(\kpick \sigma_{\kpick}(\Sigst)^2 + \tailsf_2(\roverset)\right)^2}{\sighat_r^2} +  \tailsf_1(\kpick)^2 \right).
\end{align*}



\newpage

==> body/intro_scratch <==



\paragraph{Distribution Shift v.s. Uniform Approximation} There are two prevalent perspectives on extrapolation to out-of-distribution test data.  For concreteness, let us restrict our discussion to \emph{supervised learning} - prediction of labels from covariates - and to \emph{covariate shift} - where the conditional distribution of labels given covariates is identical between test and train data.

The formidable body of empirical and theoretical work has studied covariate shift under the broader umbrella of \emph{distribution shift}. Though not an explicit assumption, many of these works implicitly regard the test and train distributions are ``close'' in some sense, for example, that the ratio between the densities of the two distributions is bounded. The challenge is how the ``distance'' between these data translates into gaps between test and train performance.

In contrast, classical statistics emphasizes settings where the conditional distribution of labels given covariates is described by a learnable (though possibly infinite dimensional ) regression function. In many settings - including classical linear regression and nonparametric estimation of H\"older smooth functions -  such a function can be approximated to uniform accuracy. Therefore, regardless of the distribution of the covariates, the labels can be predicted with near optimal accuracy.  

Real data exhibits characteristics of both the distribution shift and the uniform approximation settings. \mscomment{examples}


==> body/matrix_factorization.tex <==
%!TEX root = ../main.tex




\newpage

\subsection{Finite-Dimension Matrix Algebra} 

Given  any matrix $\bstM$ with rank $r \in \N$, we let $\bstM_r$ denote the rank-$r$ SVD of $\bstM$, and let $\bstP_r,\bstQ_r$ denote the projection to its left (resp. right) singular spaces (breaking ties arbitrarily). We denote the singular values of $\bstM$ by $\sigst_i$, and define the tail function
\begin{align*}
\tailM(r)^2 := \|\bstM - \bstM_r \|_{\fro}^2 = \sum_{i > r}(\sigst_i)^2 
\end{align*}
We assume the following risk condition
\begin{align}
\|\bhatA\bhatB^\top - \bstM\|_{\fro}^2 \le \epsrisk^2 + \inf_{\bM: \rank(\bM) = r_0}\|\bM - \bstM\|_{\fro}^2 \label{eq:risk_cond}
\end{align}
\newcommand{\errnogap}{\mathrm{Err}_{\mathrm{no,gap}}}
\begin{theorem}[Matrix factorization, no gap]\label{thm:no_gap} Fix $1 \le r < r_0 $ and $\gamma \in (0,1)$, and let $\bstM  \in \R^{n \times m}$. Suppose that $\bhatA \in \R^{n \times r_0}$ and $\bhatB \in \R^{m \times r_0}$ are balanced and satisfy \Cref{eq:risk_cond}.  Define the error term
\begin{align*}
\errnogap(\epsrisk,r,r_0) :=\frac{\epsrisk^2}{\sigst_{r_0}} +  \frac{\epsrisk \|\bstM\|_{\fro}}{ \sigst_r} + \frac{\tailM(r)^2 }{\sigst_{r_0}} +  \frac{\tailM(r_0)\|\bstM\|_{\fro}}{\sigst_{r}}
\end{align*}
Then, if (a) $\errnogap(\epsrisk,r,r_0) \le \gamma\|\bstM\|_{\fro}$, and (b) $\epsrisk \le \min\{(1-\gamma)\sigst_{r_0},(1-\gamma)\sigma_r - \sigst_{r_0+1}\}$, it holds that there exists $\bstilAr,\bstilBr$ such that $\bstilAr(\bstilBr)^\top \bstMr$ and 
\begin{align*}
\|\bhatA - \bstilAr\|_{\fro}^2 \vee \|\bhatB - \bstilBr\|_{\fro}^2  \lesssim \frac{\errnogap(\epsrisk,r,r_0)}{\gamma}.
\end{align*}
\end{theorem}

\subsection{Proof of \Cref{thm:no_gap}}



\mscomment{continue from here}
 We denote the singular values of $\bstM$ by $\sigst_i$, and define the tail function
\begin{align*}
\tailM(r)^2 := \|\bstM - \bstM_r \|_{\fro}^2 = \sum_{i > r}(\sigst_i)^2 
\end{align*}
We define the error terms $\epsfro$, $\epsop$, $\epsrisk$ via
\begin{align*}
\epsfro^2 = \|\bhatM - \bstM\|^2_{\fro}, \quad \epsop^2 = \|\bhatM - \bstM\|^2_{\op}, \quad \epsrisk^2 = \epsfro^2 - \tailM(r_0)^2.
\end{align*}
Here, $\epsfro$ and $\epsop$ capture the Frobenius and operator norm excess, whereas $\epsrisk^2$ captures the total excess square Frobenius norm error over the best rank-$r_0$ approximation. The following two estimates control $\epsop$ and $\sigma_{r_0}(\bhatM)$ in terms of $\epsrisk$:
\begin{lemma}\label{lem:epsop_lem} $\epsop \le \epsrisk + \sigma_{r_0+1}(\bstM)$.
\end{lemma}
\begin{proof} Define $\delta_i = \sigma_i(\bstM - \bhatM)$. By \Cref{lem:li_elementary}, we have that $\delta_i \ge \sigma_{r_0+i}(\bstM)$. Moreover, $\epsfro^2 = \sum_{i=1}^{\min\{n,m\}} \delta_i^2$. Therefore, 
\begin{align*}
\epsfro^2 &= \sum_{i=1}^{n \wedge m} \delta_i^2 = \delta_1^2 + \sum_{i=2}^{n \wedge m} \delta_i^2 \\
&\ge \delta_1^2+ \sum_{i=2}^{n \wedge m} \sigma_{r_0+i}(\bstM)^2\\
&= \delta_1^2 - \sigma_{r_0+1}(\bstM)^2 + \sum_{i=1}^{n \wedge m} \sigma_{r_0+i}(\bstM)\\
&=  \delta_1^2 - \sigma_{r_0+1}(\bstM)^2 + \tailM(r_0)^2. 
\end{align*}
Noting that $\delta_1 = \sigma_1(\bstM - \bhatM) = \opnorm{\bstM - \bhatM}$, we conclude $\opnorm{\bstM - \bhatM}^2 \le \sigma_{r_0+1}(\bstM)^2 + \epsfro^2 - \tailM(r_0)^2  = \sigma_{r_0+1}(\bstM)^2 + \epsrisk^2$. The bound now follows from the elementary inequality that for any $x,y \ge 0$, $\sqrt{x^2+y^2} \le x + y$.
\end{proof}

\begin{lemma}\label{lem:sig_rnot} We have $\sigma_{\rnot}(\bhatM) \ge \sigst_{\rnot} - \epsrisk$.
\end{lemma}
\begin{proof} By \Cref{lem:Mat_pert_one}, we have that
\begin{align*}
\sum_{i\ge1} (\sigma_i(\bstM) - \sigma_i(\bhatM))^2 \le \|\bstM - \bhatM\|_{\fro}^2 = \epsrisk^2 + \tailM(r_0)^2.
\end{align*}
Since $\rank(\bhatM) = r_0$, we find  $\sum_{i\ge1 } (\sigma_i(\bstM) - \sigma_i(\bhatM))^2 = \tailM(\rnot)^2 + \sum_{i=1}^{\rnot} (\sigma_i(\bstM) - \sigma_i(\bhatM))^2$. Hence, 
\begin{align*}
\sum_{i=1}^{\rnot} (\sigma_i(\bstM) - \sigma_i(\bhatM))^2 \le \epsrisk^2.
\end{align*}
In particular, $(\sigma_{\rnot}(\bstM) - \sigma_{\rnot}(\bhatM))^2  \le \epsrisk$, so that $\sigma_{\rnot}(\bhatM) \ge \sigma_{\rnot}(\bstM) - \epsrisk = \sigst_{\rnot} - \epsrisk$.
\end{proof}
We now establish that, for some $r \le \rnot$ there exists another factorization, $\bstilAr,\bstilBr$ such that $\bstilAr(\bstilBr)^\top = \bstM_r$ for which 
\begin{align*}
\bhatA \approx \bstilAr, \quad \bhatB \approx \bstilBr. 
\end{align*}
To this end, we decompose
\begin{equation}\label{eq:ortho_decomp}
\begin{aligned}
\|\bhatA - \bstilAr\|_{\fro}^2 &= \|\bstP_r(\bhatA - \bstilAr)\|_{\fro}^2 + \|(\eye_n-\bstP_r)(\bhatA -\bstilAr)\|_{\fro}^2 =\|\bstP_r\bhatA - \bstilAr\|_{\fro}^2 + \|(\eye_n-\bstP_r)\bhatA \|_{\fro}^2 \\
\|\bhatB - \bstilBr\|_{\fro} &= \|\bstQ_r(\bhatB - \bstilBr)\|_{\fro}^2 + \|(\eye_m-\bstQ_r)(\bhatB - \bstilBr)\|_{\fro}^2 = \|\bstQ_r\bhatB - \bstilBr\|_{\fro}^2 + \|(\eye_n-\bstQ_r)\bhatB \|_{\fro}^2,
\end{aligned}
\end{equation}
where above, we uses that $\bstP_r \bstilAr = \bstilAr$ and $\bstQ_r \bstilBr = \bstilBr$. 
Our first step verifies that there exists such an $\bstilAr$ and $\bstilBr$ which are close to $\bstP_r\bhatA$ and $\bstQ_r\bhatB$. 
\begin{restatable}{proposition}{propprojectedfactor}\label{prop:projected_factor} Given $\gamma \in (0,1)$, suppose $\epsop \le (1-\gamma) \sigma_r(\bstM)$.  There exists matrices $\bstilAr,\bstilBr$ such that $\bstilAr(\bstilBr)^\top = \bstM_r$ such that
 \begin{align*}
 2\|\bstP_r\bhatA  - \bstilAr\|_{\fro}^2 +  \|\bstQ_r\bhatB - \bstilBr\|_{\fro}^2 \le \frac{4\epsfro\|\bstM\|_{\fro}}{\gamma \sigma_r(\bstM)}\left(4 + \epsfro\cdot\frac{\cproc\|\bstM\|_{\op}}{\gamma\sigma_r(\bstM)\|\bstM\|_{\fro}}\right),
 \end{align*}
 where $\cproc = 1/(\sqrt{2}-1)$. 
 \end{restatable}
 Notice that, by \Cref{lem:epsop_lem}, a sufficient condition is simply that $(1-\gamma)\sigma_r(\bstM) \ge  \sigst_{r_0+1} + \epsrisk$, that is $\epsrisk \le (1-\gamma)\sigma_r - \sigst_{r_0+1}$. Further, for $\epsfro \le \frac{\gamma\|\bstM\|_{\fro}\sigma_r(\bstM)}{\|\bstM\|_{\op}}$, the above simplifies to
  \begin{align*}
 2\|\bstP_r\bhatA  - \bstilAr\|_{\fro}^2 +  \|\bstQ_r\bhatB - \bstilBr\|_{\fro}^2 \le \frac{(16 + 4\cproc)\epsfro\|\bstM\|_{\fro}}{\gamma \sigma_r(\bstM)^2}
 \end{align*} 

 \begin{restatable}{proposition}{offpropprojectedfactor}\label{prop:off_projected_factor}
The following bound holds:
 \begin{align*}
\fronorm{(\eye_n - \bstP_r)\bhatA}^2 \vee \fronorm{\bhatB(\eye_m - \bstQ_r)}^2 \le \frac{7\epsfro^2 +  2\tailM(r)^2 }{\sigma_{r_0}(\bhatM)} \le \frac{7\epsrisk^2 +  9\tailM(r)^2 }{\sigma_{r_0}(\bhatM)}
\end{align*}
Invoking \Cref{lem:sig_rnot}, as soon as $\epsrisk \le (1-\gamma)\sigst_{r_0}$, 
\begin{align*}
\fronorm{(\eye_n - \bstP_r)\bhatA}^2 \vee \fronorm{\bhatB(\eye_m - \bstQ_r)}^2 \le\frac{7\epsrisk^2 +  9\tailM(r)^2 }{\gamma \sigst_{r_0}}
\end{align*}
\end{restatable}
Hence, we from \Cref{eq:ortho_decomp} and the above two propositions, we find that if $ \epsrisk \le \min\{(1-\gamma)\sigst_{r_0},(1-\gamma)\sigma_r - \sigst_{r_0+1}\}$ and $\epsfro \le \frac{\gamma\|\bstM\|_{\fro}\sigma_r(\bstM)}{\|\bstM\|_{\op}}$, 
\begin{align*}
\|\bhatA - \bstilAr\|_{\fro}^2 \vee \|\bhatB - \bstilBr\|_{\fro}^2 &\le \frac{7\epsrisk^2 +  9\tailM(r)^2 }{\gamma\sigst_{r_0}} + \frac{(16 + 4\cproc)\epsfro \|\bstM\|_{\fro}}{\gamma \sigst_r}\\
&\le \frac{7\epsrisk^2 +  9\tailM(r)^2 }{\gamma\sigst_{r_0}} + \frac{(16 + 4\cproc)\epsfro \|\bstM\|_{\fro}}{\gamma \sigst_r}\\
&\lesssim \frac{1}{\gamma}\left(\frac{\epsrisk^2}{\sigst_{r_0}} +  \frac{\epsrisk \|\bstM\|_{\fro}}{ \sigst_r} + \frac{\tailM(r)^2 }{\sigst_{r_0}} +  \frac{\tailM(r_0)\|\bstM\|_{\fro}}{\sigst_{r}}\right) \\
&:= \mathrm{Err}(\epsrisk,r,r_0,\gamma)
\end{align*}
Lastly, the condition $\epsfro \le \frac{\gamma\|\bstM\|_{\fro}\sigma_r(\bstM)}{\|\bstM\|_{\op}}$ holds as soon as $\epsfro \le \gamma\sigma_r(\bstM)$, which holds as soon as $\mathrm{Err}(\gamma,\epsrisk,r,r_0) \le  \|\bstM\|_{\fro}$.


\subsection{Procrustes Lemma}
\begin{lemma}\label{lem:proc} Let $(\bX_1,\bY_1)$ and $(\bX_2,\bY_2)$ be rank-$r$ balanced factorization of matrices $\bM_1$ and $\bM_2$, respectively. Suppose that $\|\bM_1 - \bM_2\|_{\op} \le (1-\gamma)\|\bM_1\|_{\op}$. Then, there exist an orthogonal matrix $\bO \in \bbO(r)$ such that
\begin{align*}
\|\bX_1 - \bX_2 \bO\|_{\fro}^2 + \|\bY_1 - \bY_2 \bO\|_{\fro}^2 \le \cproc \frac{\|\bM_1 - \bM_2\|_{\fro}^2}{\gamma \sigma_r(\bM_1)}, 
\end{align*} 
where $\cproc =\frac{1}{\sqrt{2}-1}$. 
\end{lemma}
\begin{proof}[Proof Sketch] The proof is nearly indentical to that of \mscomment{Lemma 5.14}. The only differences are that, when tracing the proof (a), we have 
\begin{align*}
\sigma_{2r}\left(\begin{bmatrix} \bX_1 & \bX_2 \\ - \bY_1 & -\bY_2 \end{bmatrix}\begin{bmatrix} \bX_1 & \bX_2 \\ - \bY_1 & -\bY_2 \end{bmatrix}^\top\right) \ge \sigma_r(\bM_1) - (1-\gamma)\sigma_{r}(\bM_1) = \gamma \sigma_{r}(\bM_1),
\end{align*}
and that (b), we terminate the proof at the second-to-last inequality (rather than recasting in terms of the $\mathrm{dist}$ function defined therein). 
\end{proof}
\subsection{Regression with corrupted covariances}

\begin{lemma}
Let $\cD$ be a joint distribution over random variables $(x,y,z)$such that $z = h_{\star}(x,y)$.  Then, for any functions $\ftilst: \cX \to \hilspace$, $\gtilst: \cY \to \hilspace$, Then,
\begin{align*}
\Exp[\langle \ftilst(x), \ghat(y) - \gtilst(y)\rangle^2] &\le 2\Exp[(\langle \fhat(x), \ghat(y)\rangle - z)^2 ]  + 4B^2\Exp[\|\fhat - \ftilst(x)\|^2]  + 4 \Exp[(\langle \ftilst(x),\gtilst(y)\rangle - h_{\star}(x,y))^2 ]
\end{align*}
\end{lemma}
\newcommand{\sfP}{\mathsf{P}}
\newcommand{\fchst}{\check{f}^\star}
\newcommand{\gchst}{\check{g}^\star}
\newcommand{\echst}{\check{e}^\star}








==> body/old_body.tex <==

\mscomment{explain the proof}


\newpage
\paragraph{Eigengap:}

We decompose these errors via the following
\begin{lemma}[Key Matrix Error Decomposition]\label{lem:matdecomp_weighted} Fix ranks $r,r_1 \in \N$. Let $\bR \in \GL{r_0}$, and let $\bA = \bhatA \bR$, and $\bB = \bhatB \bR^{-\top}$, so that $\bhatM = \bA\bB^\top$. Then, 
\begin{align*}
\ErrTerm_0(\bA,\bB)  \le 10 \mu(\bR)^2 T_1\cdot( \|\bstM\|_{\op} +\|\bstM - \bhatM\|_{\op} ) + 8T_2 + 2T_3,
\end{align*}
where $\mu(\bR) := \max\{\opnorm{\bR},\opnorm{\bR^{-1}}\}$, and where we define the matrix error terms:
\begin{align}
T_1 = T_1(\bA,\bB;k,r_1) &:= \|\bstPk\bhatP_{r_1}\bA - \bstAk\|_{\fro}^2 + \|\bstQk\bhatQ_{r_1}\bB - \bstBk\|_{\fro}^2 \label{eq:T_one}\\
T_2 = T_2(r_1)  &:= \|\bhatM_{>r_1}\|_{\fro}^2\label{eq:T_two}\\
T_3 = T_{3}(k) &:= \|(\eye_n-\bstPk)\bhatM\|_{\fro}^2 \vee  \|\bhatM(\eye_m-\bstQk)\|_{\fro}^2\label{eq:T_three}. 
\end{align}
\end{lemma}

\mscomment{fix this so that $\bhatA,\bhatB$ is approximately balanced:}

Terms $T_2$ and $T_3$ are straightforward to bound (see \Cref{app:t2_t3}):
\begin{lemma}\label{lem:t2_bound} For any $r \in \N$, $T_2(r_1) \le 2\epsfro^2 + 2\epsapx(r_1)$. 
\end{lemma}
\begin{lemma}\label{lem:t3_bound} For $r \in \N$,  $T_3(k) \le 2\epsfro^2 + 2\epsapx(k)$. In particular, if $r_1 \ge k$, then
\begin{align*} T_2(r_1) + T_3(k) \le 4\epsfro^2 + 4\epsapx(k). 
\end{align*}
Alternatively, $T_3$ also satisfies $T_3(k) \le \|\bhatM - \bstMk\|_{\fro}^2 $. 
\end{lemma}

\subsection{}

 \begin{restatable}{lemma}{wedinapply}\label{lem:wedin_closeness_aplied} Suppose that $\frac{\|\bhatM - \bstM\|_{\op}}{\sigma_{k}(\bstM) } \le \delstk/6$. Then, the following are true:
    \begin{itemize}
        \item[(a)] $ \|\bstPk\bhatM_{k}\bstQk - \bstMk\|_{\fro} \le \frac{4}{\delstk}\|\bhatM - \bstM\|_{\fro}$
        \item[(b)] $\|\bstPk\bhatM_{k}\bstQk - \bstMk\|_{\op} \le \frac{2}{3}\sigma_k(\bstM).$
        \item[(c)] Both $(\bstPk \bhatA_{k})^\top (\bstPk \bhatA_{k})\succeq \frac{1}{5}\bhatA_k^\top \bhatA_k$ and $(\bstQk \bhatB_{k})^\top (\bstQk \bhatB_{k}) \succeq \frac{1}{5}\bhatB_k^\top \bhatB_k$. Moreover, $\rank(\bstPk \bhatA_{k}) = \rank(\bstQk \bhatB_{k}) = k$. 
    \end{itemize}
    \end{restatable}

\begin{restatable}{lemma}{lemtilbalance}\label{lem:balanced_thing_of_terms}  Suppose that $\frac{\|\bhatM - \bstM\|_{\op}}{\sigma_{k}(\bstM) } \le \delstk/6$.  There exist a $\btilA_k \in \R^{n \times k},\btilB_k \in \R^{m \times k}$ and $\btilR_k \in \GL{k}$ for which
    \begin{itemize}
        \item[(a)] $(\btilA_k,\btilB_k)$ are balanced, and $\btilA_k\btilB_k^\top = \bstPk\bhatM_{k}\bstQk$
        \item[(b)] $\btilA_k \btilR_k = \bstP_k\bhatA_k$ and $ \btilB_k \btilR_k^{-\top} = \bstQ_k\bhatB_k$
        \item[(c)] $\mu(\btilR_k)^2 := \max\{\opnorm{\btilR_k},\opnorm{\btilR_k^{-1}}\}^2 \le \sqrt{5}$.
    \end{itemize}
    \end{restatable}

   \mscomment{complete this proof}
\subsection{Bounds with gaps}

\begin{lemma} Suppose $\|\bhatM - \bstMk\| \le \dots$. Then, $\|\bhatM_k - \bstM_k\| \le \dots$. 
\end{lemma}


\mscomment{TODOs
\begin{itemize}
	\item Instantiate Gaps
	\item Explain how small $\epsop$ has to be
	\item err
\end{itemize}}
\begin{lemma}
\end{lemma}

\subsection{Factor Error}

\begin{restatable}[Key Matrix Error Decomposition]{lemma}{matdecomp}\label{lem:factor_decomp}
\begin{align*}
\ErrTerm_1 \le \|\bhatA - \bstA_r\|_{\fro}^2 + \|\bhatB - \bstB_r\|_{\fro}^2 &\le \dots
\end{align*}
where $T_1$ is as in \Cref{eq:T_one}, and where \mscomment{todo}.
\end{restatable}



==> body/proof_corollaries.tex <==
%!TEX root = ../main.tex
\section{Proof of ??}


\subsection{Proof of \Cref{cor:double_train,cor:sing_train}}

Throughout, we recall that \Cref{defn:error_regimes} lays out the constants for the good, good single-training, and good double-training regimes.  Before proving the corollaries, we have the following estimate.
\begin{claim}\label{claim:good_regime} In a good regime, we have
\begin{align*}
\tailsf_2(r) \le \Psitwo(r_0) +  \cpsi^2 r_0\psi(r_0)^2, \quad \tailsf_1(r)  \le \Psione(r_0) + \cpsi r_0\psi(r_0)
\end{align*}
\end{claim}
\begin{proof} We bound $\tailsf_2(r)$; the computation for $\tailsf_1(r)$ is similar.
\begin{align*}
\tailsf_2(r) = \sum_{ n > r} (\sigst_n)^2  &= \sum_{n > r_0} (\sigst_n)^2  + \sum_{n=r+1}^{r_0} (\sigst_n)^2 \\
&\le \Psitwo(r_0) + r_0 (\sigst_r)^2 \\
&\le \Psitwo(r_0) + \cpsi^2 r_0\psi(r_0)^2.
\end{align*}
\end{proof}


\begin{proof}[Proof of \Cref{cor:sing_train}, good single-training regime]. Let $\epsilon^2 := \max\{\epsone^2, \epstrain^2\}$ so that 
\begin{align*}
\Risk(\fhat,\ghat;\Dtest) &\lesssim_{\star}    \alpha_0\left(\left\{r^4 \epsilon^2  +  \tailsf_1(r)^2 + r^2 (\bsigst_{r+1})^2 \right\}  +   \left\{\frac{r^6 \epsilon^4 +  \tailsf_2(r)^2 }{(\bsigst_r)^2}     \right\}\right).    
\end{align*}
In a good single-trailing regime, we have $\epsilon^2 \le \csint(\alphatrain \tailsf_2(r) + \betrain)$. Using that $\csint,\alphatrain \ge 1$, our upper bound on $\epsilon^2$  dominates $\tailsf_2(r)$. Thus, 
\begin{align*}
&\Risk(\fhat,\ghat;\Dtest) \\
&\lesssim_{\star}    \alpha_0\left(\left\{\csint(\alphatrain \tailsf_2(r) + \betrain)  +  \tailsf_1(r)^2 + r^2 (\bsigst_{r+1})^2 \right\}  +   \left\{\frac{r^6 \csint^2(\alphatrain^2 \tailsf_2(r)^2 + \betrain^2)  }{(\bsigst_r)^2}     \right\}\right)\\
&\lesssim_{\star}    \alpha_0\left(\left\{\csint(\alphatrain \tailsf_2(r) + \betrain)  +  \tailsf_1(r)^2 + r^2 (\bsigst_{r+1})^2 \right\}  +   \left\{\frac{\csint^2r^6 (\alphatrain^2 \tailsf_2(r)^2 + \betrain^2)  }{\psi(r_0)^2}     \right\}\right)\\
&\lesssim_{\star}    \alpha_0\left(\underbrace{\left\{\csint\alphatrain \tailsf_2(r)  +  \tailsf_1(r)^2 + r^2 (\bsigst_{r+1})^2 \right\}}_{(\star)}  +   \underbrace{\left\{\frac{\csint^2 \alphatrain^2 r^6  \tailsf_2(r)^2   }{\psi(r_0)^2}     \right\}}_{(\star \star)}\right) \\
&\quad+ \alpha_0\left(\underbrace{\csint \betasint +\frac{r^6  \csint^2 }{\psi(r_0)^2}\cdot\betasint^2}_{\Ferrst}\right)
\end{align*}
To bound $(\star)$, we first use $\csint,\alphatrain \ge 1$ and $\tailsf_1(r)^2 \ge \tailsf_2(r)$, and well as $\bsigst_{r+1} \le \cpsi \psi(r_0)$, followed by \Cref{claim:good_regime} to bound
\begin{align*}
\csint\alphatrain \tailsf_2(r)  +  \tailsf_1(r)^2 + r^2 (\bsigst_{r+1})^2 &\lesssim \csint\alphatrain \tailsf_1(r)^2 + r^2 \cpsi^2 \psi(r_0)^2\\
&\lesssim \csint\alphatrain (\Psione(r_0)^2 + r_0^2 \cpsi^2 \psi(r_0)^2) +  r^2 \cpsi^2 \psi(r_0)^2 \\
&\lesssim \csint\alphatrain (\Psione(r_0)^2 + r_0^2 \cpsi^2 \psi(r_0)^2). 
\end{align*}
To bound $(\star \star)$, we take
\begin{align*}
\csint^2 \alphatrain^2 r^6 \frac{  \tailsf_2(r)^2   }{\psi(r_0)^2}  &\lesssim\csint^2 \alphatrain^2 r^6 \left\{ \frac{  \Psitwo(r_0)^2  + \cpsi^2 r_0^2 \psi(r_0)^4 }{\psi(r_0)^2}\right\} \\
&= \csint^2 \alphatrain^2 r^6\left\{\frac{  \Psitwo(r_0)^2  }{\psi(r_0)^2}  + \cpsi^2 r_0^2 \psi(r_0)^2\right\}.
\end{align*}
Hence, using  $\cpsi^2 \csint^2 \alphatrain^2 r^6 \ge 1$,  
\begin{align*}
(\star) + (\star \star) \lesssim \csint\alphatrain \Psione(r_0)  + \csint^2 \alphatrain^2 r^6\left\{\frac{  \Psitwo(r_0)^2  }{\psi(r_0)^2}  + \cpsi^4 r_0^2 \psi(r_0)^2\right\}\\
\lesssim   \csint^2 \alphatrain^2 r^6\underbrace{\left\{ \Psione(r_0)^2 + \frac{  \Psitwo(r_0)^2  }{\psi(r_0)^2}  + \cpsi^4 r_0^2 \psi(r_0)^2\right\}}_{\frakFtrain}
\end{align*}
concluding the proof.
\end{proof}

\begin{proof}[Proof of \Cref{cor:double_train}] As shorthand, define $\frakF$ such that $\Risk(\fhat,\ghat;\Dtest) \lesssimst \alpha_0 \frakF$, that is, take
\begin{align*}
\frakF := \left(  \left(r^4 \epsone^2 +  \epstrain^2  +  \tailsf_1(r)^2 + r^2 (\bsigst_{r+1})^2 \right)  +  \frac{r^6 \epsone^4 + \epstrain^4  +  \tailsf_2(r)^2 }{(\bsigst_r)^2}     \right).
\end{align*} 
Invoking the definition of a good double training regime (again, \Cref{defn:error_regimes}),
\begin{align*}
\frakF &\lesssim  r^4\alphadt \Psitwo(\pdub)  + \alphtrain \tailsf_2(r) + \tailsf_1(r)^2 + \cpsi^2 r^2 \psi(r_0)^2 + \frac{r^6 \alphadt^2 \Psitwo(p_1)^2 + (\alphatrain^2+1) \tailsf_2(r)^2 }{(\bsigst_r)^2} \\
&\quad + r^4 \betadt + \betrain + (r^6 \betadt^2 + \betrain^2)/(\bsigst_r)^2 \\
&\lesssim  \underbrace{r^4\alphadt \Psitwo(\pdub)  + \alphtrain \tailsf_2(r) + \tailsf_1(r)^2 + \cpsi^2 r^2 \psi(r_0+1)^2}_{(\star)} +  \cdot \underbrace{ \frac{r^6 \alphadt^2 \Psitwo(\pdub)^2 + \alphatrain^2 \tailsf_2(r)^2 }{\psi(r_0)^2}}_{(\star\star)} \\
&\quad + \underbrace{(r^4 \betadt + \betrain) + \frac{1}{\psi(r_0)^2} \cdot ( r^6\betadt^2 + \betrain^2)}_{ \Fdterr}
%&\quad\\
%
%&\lesssim_{\star}  \left((r+\kpick^4)\alpha_3 \tailsf_2(p) + \kpick^2 (\bsigst_{r})^2  +  \tailsf_1(\kpick)^2\right)  + \frac{\kpick^6 \alpha_2^2 \tailsf_2(r)^2 + \kpick^2 (\bsigst_{\kpick})^4 +  \tailsf_2(\kpick)^2}{\alpha_1(\bsigst_r)^2}    
\end{align*}

Hence, using $\alphatrain \ge 1$,
\begin{align*}
(\star) &\lesssim  r^4\alphadt \Psitwo(\pdub)  + \alphtrain (\Psitwo(r_0) +  \cpsi^2 r_0\psi(r_0)^2) + ((\Psione(r_0) + \cpsi r_0\psi(r_0))^2 + \cpsi^2 r^2 \psi(r_0)^2 \\
&\lesssim r^4\alphadt \Psitwo(\pdub) + \Psione(r_0)^2  + \alphatrain\{ \Psitwo(r_0) + r_0^2  \cpsi^2\psi(r_0)^2\}.
\end{align*}
Next, 
\begin{align*}
(\star\star) &=  \cdot \frac{r^6 \alphadt^2 \Psitwo(\pdub)^2 + \alphatrain^2 \tailsf_2(r)^2 }{\psi(r_0)^2} \\
&\le \frac{ r^6 \alphadt^2 \Psitwo(\pdub)^2}{\psi(r_0)^2} + \frac{ \alphatrain^2 (\Psitwo(r_0) + \cpsi^2 r_0 \psi(r_0)^2)^2}{\psi(r_0)^2} %&\lesssim c_0^2\left(\frac{r^6 \alpha_1^2 \Psitwo(p_1)^2 + c_0^2\alphatrain^2 c_1^2\Psitwo(r_0)^2 }{\psi(r_0)^2} + \alphatrain^2 c_1^2 r_0^2 \psi(r_0)^2 \right).
\end{align*}
Noting that $\alphatrain \ge 1$, we have 
\begin{align*}
\frac{ \alphatrain^2 (\Psitwo(r_0) + \cpsi^2 r_0 \psi(r_0)^2)^2}{\psi(r_0)^2}  \ge \alphatrain\{ \Psitwo(r_0) + r_0^2  \cpsi^2\psi(r_0)^2\}.
\end{align*}
Hence,
\begin{align*}
&(\star) + (\star \star)\\
&\lesssim \underbrace{r^4\alphadt \Psitwo(\pdub) + \frac{ r^6 \alphadt^2 \Psitwo(\pdub)^2}{\psi(r_0)^2}}_{\Fdtone} + \Psione(r_0)+ \frac{ \alphatrain^2 (\Psitwo(r_0) + \cpsi^2 r_0 \psi(r_0)^2)^2}{\psi(r_0)^2}\\
&\lesssim \Fdtone + \Psione(r_0)^2+  \alphatrain^2 \cdot \left\{\frac{ \Psitwo(r_0)^2 }{\psi(r_0)^2} + \cpsi^4 r_0^2 \psi(r_0^2)\right\}\\
&\le \Fdtone + \alphatrain^2  \underbrace{  \left\{\Psione(r_0)^2 + \frac{ \Psitwo(r_0)^2 }{\psi(r_0)^2} + \cpsi^4 r_0^2 \psi(r_0^2)\right\}}_{\frakFtrain}. 
\end{align*}
To summarize, we have shown
\begin{align*}
\Risk(\fhat,\ghat;\Dtest) \lesssimst \alpha_0 \frakF \lesssimst \alpha_0(\frakFtrain + \Fdtone + \Fdterr)
\end{align*}



\end{proof}
	\subsection{Proof of \Cref{lem:decay_lem}}

We begin with some standard tail bounds, which we check at the end of the section.
\begin{lemma}[Tail Bounds]\label{lem:tail_bounds} The following bounds hold
\begin{itemize}
    \item Let $\psi(n) = Cn^{-1-\gamma}$. Then, $ \Psitwo(n) \le C^2 n^{-(1+2\gamma)}$ and $\Psione(n) \le \gamma^{-1}C n^{-\gamma}$
    \item Let $\psi(n) = C\exp(-\gamma n)$. Then $\Psitwo(n) \le \frac{C^2\exp(-2\gamma n)}{\gamma}$, $\Psitwo(n) \le \frac{C\exp(-\gamma n)}{\gamma}$.
\end{itemize}
\end{lemma}
We now turn to the proof of the main lemma.
\begin{proof}[Proof of \Cref{lem:decay_lem}] Let us start with $\frakFtrain$ with  polynomial decay. For $\frakFtrain$, we have
\begin{align*}
\frakFtrain &:= \cpsi^4  \alphatrain^2\left\{ \Psione(r_0)^2 + \frac{  \Psitwo(r_0)^2  }{\psi(r_0)^2}  +  r_0^2 \psi(r_0)^2\right\}\\
&= \cpsi^4  \alphatrain^2\left\{ \gamma^{-2}C^2 r_0^{-2\gamma} +   +  \frac{C^4 r_0^{-2-4\gamma}}{C^2 r_0^{-2-2\gamma}} +  C^2 r_0^{-2(1+\gamma)}r_0^2\right\}\\
&= \cpsi^4  \alphatrain^2 \cdot(2+\gamma^{-2}) C^2 r_0^{-2\gamma}.
\end{align*}
With exponential decay, 
\begin{align*}
\frakFtrain &= \cpsi^4  \alphatrain^2\left\{ \gamma^{-2}C^2 \exp(-2r_0\gamma) +    \frac{\gamma^{-2}C^2 \exp(-4r_0\gamma) }{\exp(-2r_0\gamma)} +  C^2 \exp(- 2_0 \gamma) r_0^2\right\}\\
&= \cpsi^4 \alphatrain^2 \cdot C^2 (r_0^2+2\gamma^{-1})e^{-2\gamma r_0}.
\end{align*}
Next, we turn to $\Fdtone$. Since $r \le r_0$,we have under polynomial decay
\begin{align*}
\Fdtone \le r^4\alphadt \Psitwo(\pdub) +  \alphadt^2 \cdot \frac{ r^6\Psitwo(\pdub)^2}{\psi(r_0)^2} &= C^2 \alphadt r^4\pdub^{-1-2\gamma}\left( 1+  \alphadt \frac{ C^4 r^2\pdub^{-1-2\gamma}}{C^2 r_0^{-2-2\gamma}}\right)\\
&\le C^2\alphadt r^4\pdub^{-1-2\gamma}\left(1 +  \alphadt  r_0^{4+2\gamma}\pdub^{-1-2\gamma}\right).
\end{align*}
In particular, if $\pdub \ge r_0^2( \alphadt)^{\frac{1}{1+2\gamma}}$, then $\Fdtone \le 2C^2\alphadt r^4\pdub^{-1-2\gamma}$, and otherwise, $\Fdtone \le C^2\alphadt^2  \cdot r_0^{8+\gamma} \pdub^{-2-4\gamma}$.

Under exponential decay, 
\begin{align*}
\Fdtone \le r^4\alphadt \Psitwo(\pdub) +   \alphadt^2 \cdot \frac{ r^6\Psitwo(\pdub)^2}{\psi(r_0)^2} &= C^2 \alphadt \gamma^{-1} r^4e^{-p\gamma}\left(1 +   \alphadt \gamma^{-1}\frac{ r^2\pdub^{-2\gamma p}}{\exp(-2\gamma r_0} \right)\\
&= C^2 \alphadt \gamma^{-1} r^4e^{-p\gamma}\left(1 +   \alphadt \gamma^{-1} r^2 \exp(-2\gamma(p-r_0))\right).
\end{align*}
In particular, if $p \ge r_0 + \frac{\log( \alphadt \gamma^{-1} r^2 )}{2\gamma}$, then, $\Fdtone \le C^2 \alphadt \gamma^{-1} r^4e^{-p\gamma}$.
\end{proof}

	\begin{proof}[Proof of \Cref{lem:tail_bounds}] Let $\psi(n)$ be a non-increasing function. Then, 
	\begin{align*}
	\sum_{n \ge k+1} \psi(n) &=  \sum_{n \ge k+1} \int_{n-1}^n\psi(t)\rmd t \le  \int_{k}^{\infty}\psi(t)\rmd t.
	\end{align*}
	Now, if  $\Sigst$ has $(C,\gamma)$-polynomial decay, then 
	\begin{align*}
	\Psitwo(n) &= \sum_{k \ge n+1}\psi(k) \le C^2\sum_{k \ge n+1}k^{-2(1+\gamma)} \le C^2\int_{n}^{\infty}t^{-(2+2\gamma)}\rmd t = \frac{C^2 n^{-(1+2\gamma)}}{(1+2\gamma)} \le C^2 n^{-(1+2\gamma)},
	\end{align*}
	where above we use $\gamma > 0$.  By a similar computation
	\begin{align*}
	\Psione(n) \le C\int_{n}^{\infty}t^{-(1+2\gamma)}\rmd t \le \frac{Cn^{-\gamma}}{\gamma }.
	\end{align*}
	Under exponential decay, 
	\begin{align*}
	\Psitwo(n)&\le  C^2\int_{n}^{\infty}\exp(-2\gamma t)\rmd t \le \frac{C^2}{2\gamma}\exp(-2\gamma n) \le C^2\gamma^{-1}\exp(-2\gamma n)
	\end{align*}
	Similarly, $\Psione(n) \le \frac{C\exp(-\gamma n)}{\gamma}$.
	\end{proof}


\begin{comment}
\subsection{Proof of \Cref{lem:errbar_train}}
	 By Assumption ????, we have
	\begin{align*}
	\errtrain &\le \epstrain + \alphatrain\Risk(\fst_r,\gst_r;\Dtrain).
	\end{align*}
	Moreover, arguing as in \Cref{lem:risk_decomp_one}, we can bound 
	\begin{align*}
	\Risk(\fst_r,\gst_r;\Dtrain) &\le \kapdens \sum_{i,j \in \{1,2\}}\alphatrain\Risk(\fst_r,\gst_r;\disij)\\
	&\le \kapdens (1+\kapcov)^2 \Risk(\fst_r,\gst_r;\cD_{1\otimes 1})\\
	&\overset{(ii)}{=} \kapdens (1+\kapcov)^2 \tailsf_2(r).
	\end{align*}
	where in $(i)$  we use \Cref{claim:ij_to_train} and in $(ii)$ we use \Cref{lem:tailsf_two}. Hence, we can take 
	\begin{align*}
	\errtrain &\le \epstrain + \alphatrain\kapdens(1+\kapcov)^2\tailsf(r) =:\errbartrain. 
	\end{align*}
	The result follows from using $\kapcov \ge 1$.
	\qed

	\subsection{Proof of \Cref{thm:granular_error_bound}}
	Set $\errbartrain := \epstrain + \alphatrain\kapdens(1+\kapcov)^2\tailsf(r)$. By \Cref{lem:errbar_train}, we have  $\errbartrain \ge \errtrain$. Further,  by \Cref{claim:ij_to_train}, $\errbartrain/\omegaoff \ge \Risk(f,g;\cD_{1\otimes 1})$. Hence, applying \Cref{thm:one_block} with $\epsilon^2 \gets \epstrain$, we see that
	\begin{align*}
	s^2 < \frac{ \omegaoff\|\Sigst\|_{\op}^2}{1600\errbartrain},
	\end{align*}
	there are functions $(f,g)$ which are $(\sighat_r,r)$-strongly-supported and compatible with $\projopstk$, and satisfy. 
	\begin{align*}
	\frac{(\ErrTerm_0(f,g,k) + \errapx(k) +  (\errtrain /\omegaoff))^2}{\sighat_r^2}  &\lesssim \frac{s^6 }{\sighat_r^2}\frac{\errbartrain^2}{\omegaoff^2} + \frac{\left(\kpick \sigma_{\kpick}(\Sigst)^2 + \tailsf_2(s)\right)^2}{\sighat_r^2}\\
	\ErrTerm_1(f,g,k)^2 &\lesssim (r+\kpick^4) \frac{\errbartrain}{\omegaoff}+ \kpick^2 \sigma_{\kpick}(\Sigst)^2  +  \tailsf_1(\kpick)^2
	\end{align*}
	Since $\sighat_r \le \sigma_{r}(\Sigst) \le \sigma_{\kpick}(\Sigst)$, we have $\kpick^2 \sigma_{\kpick}(\Sigst)^2 \le \frac{(\kpick \sigma_{\kpick}(\Sigst)^2 + \tailsf_2(s))^2}{\sighat_r^2} + \frac{(\kpick \sigma_{\kpick}(\Sigst)^2 + \tailsf_2(s))^2}{\sighat_r^2}$. Hence, 
	\begin{align*}
	&\ErrTerm_1(f,g,k)^2 + \frac{(\ErrTerm_0(f,g,k) + \errapx(k) +  (\errtrain /\omegaoff))^2}{\sighat_r^2} \\
	&\lesssim  (r+\kpick^4)\frac{\errbartrain}{\omegaoff}+ \frac{s^6 }{\sighat_r^2}\frac{\errbartrain^2}{\omegaoff^2} + \frac{\left(\kpick \sigma_{\kpick}(\Sigst)^2 + \tailsf_2(s)\right)^2}{\sighat_r^2} +  \tailsf_1(\kpick)^2. 
	\end{align*}
	Again, since $k \ge r$, $\sighat_r^2 \le \sigma_r(\Sigst)^2 \le \tailsf_2(k) = \errapx(k)$ by \Cref{lem:tailsf_two}. Since, we can invoke \Cref{prop:final_error_decomp} to bound $\Risk(f,g;\Dtest)/\kapdens$ by 
	\begin{align*}
	&\lesssim \omega_{22}\kapcov^2\left((r+\kpick^4)\frac{\errbartrain}{\omegaoff} + \frac{s^6 }{\sighat_r^2}\frac{\errbartrain^2}{\omegaoff^2} + \frac{\left(\kpick \sigma_{\kpick}(\Sigst)^2 + \tailsf_2(s)\right)^2}{\sighat_r^2} +  \tailsf_1(\kpick)^2. \right) \\
	&\quad + (1 + \frac{\kapcov\omega_{22}}{\omegaoff}) \errtrain.
	\end{align*}
	Using $\kapcov \ge 1$ and $\epstrain \le \errbartrain$, the second term on the last line can be absorded into the first . Thus, we can bound $\Risk(f,g;\Dtest)/\kapdens$ by 
	\begin{align*}
	&\lesssim \errbartrain +  \omega_{22}\kapcov^2\left((r+\kpick^4)\frac{\errbartrain}{\omegaoff} + \frac{s^6 }{\sighat_r^2}\frac{\errbartrain^2}{\omegaoff^2} + \frac{\left(\kpick \sigma_{\kpick}(\Sigst)^2 + \tailsf_2(s)\right)^2}{\sighat_r^2} +  \tailsf_1(\kpick)^2 \right). 
	\end{align*}
	\qed
\end{comment}

==> body/setup.tex <==
%!TEX root = ../main.tex

\section{Motivation}
The goal here is to leverage the training set to not just learn a model that generalizes to new samples drawn from the \emph{same} training distribution, but instead to learn a model that is able to leverage the training set to learn the relationship between different subsets of the training data and use this to potentially deal with distribution shift at test time. The change in assumption becomes \textemdash rather than assuming the test distribution $p_{\text{test}}(x, y)$ is the same as the training distribution $p_{\text{train}}(x, y)$, the difference (used loosely) between train and test distributions needs to be within the distribution of differences between subdistributions of the training set. By shifting the burden of generalization to the difference rather than the training distrbution itself, there is a potential to generalize to distributions outside the training set. 


\section{Formulation}
To formulate this problem setting, let us consider a goal conditioned imitation learning problem. Let's say the training distribution is a set of optimal trajectories starting from the origin and going to different goals as shown in Figure  \ref{fig:traindist}.  

\begin{figure}[!h]
    \centering
    \includegraphics[width=0.35\linewidth]{figs/training_dist.png}
    \caption{Training distribution}
    \label{fig:traindist}
\end{figure}

The training dataset consists of trajectories $\mathcal{D} = \{s_0^i, a_0^i, s_1^i, a_1^i, \dots, s_T^i, a_T^i, g^i\}_{i=1}^N$ where the goals are drawn from some distribution of goals $p_{\text{train}}(g)$ and the trajectories optimally reach the goals. A standard imitation learning objective would optimize a standard supervised learning objective like 
 
\kz{would written in the log-likelihood be  slightly more sensible?}
\begin{equation}
    \max_{\theta} \mathbb{E}_{(s, a, g) \sim \mathcal{D}}\left[ \pi_{\theta}(a|s, g) \right]
\end{equation}

This performs well on new testing goals also drawn from $p_{\text{train}}(g)$ as shown below in Fig [], but fails to do well on goals drawn from a different distribution $p_{\text{test}}(g)$ as shown in Fig []. The problem we're going to try and solve is how we can leverage the training set to improve the performance on at least choices types of  $p_{\text{test}}(g)$. 


\begin{figure}[!h]
    \centering
    \includegraphics[width=0.35\linewidth]{figs/indist.png}
    \caption{Performance on in distribution points}
    \label{fig:indist}
\end{figure}


\begin{figure}[!h]
    \centering
    \includegraphics[width=0.35\linewidth]{figs/outdist.png}
    \caption{Performance on out of distribution points}
    \label{fig:ood}
\end{figure}

The key insight we are going to take is that we can use the training set to simulate distribution shift and learn residual models that can modify behavior of a model trained on a particular distribution $p_{\text{train}}(g)$ to be good on $p_{\text{test}}(g)$ subject to knowing what the difference between the distributions actually is. In this instantiation we are actually going to do this at the instance level, i.e we are going to say that for a new $g_{\text{test}} \sim p_{\text{test}}(g)$, where the model may perform poorly, we are going to modify a behavior of an ``in-distribution" point using a residual model to get good ``out-of-distribution" behavior. 

So let us say we have trained a goal conditioned imitation model \kz{maybe introduce the parameterized form with  $\theta$ to make it consistent.} $\pi(a|s, g): \mathcal{S} \times \mathcal{G} \rightarrow \mathcal{A}$ as described in Eqn [], we can then learn a residual transformation model $g_\phi(a'|a, \delta(g)): \mathcal{A} \times \mathcal{G} \rightarrow \mathcal{A}$. This residual is trained on pairs of $g$, $g'$ sampled from the training distribution. \kz{using $g$ ($g_\phi$ and $g$) for both transformation model and goal might be confusing.}\kz{why not $g_\phi(a'|s,g, \delta(g))$?}

So, given a sampling distribution $p(i, j)$ which samples pairs of datapoint indices $i, j$ from the training distribution corresponding to goals $g_i, g_j$, the residual policy is trained via the following objective. 

\begin{equation}
    \max_{\phi} \mathbb{E}_{(i, j) \sim p(i, j), (s_t^i, a_t^i, g^i), (s_t^j, a_t^j, g^j) \sim \mathcal{D}}\left[ g_{\phi}(a_t^j|\pi_\theta(.|s, g_i), g_j - g_i) \right]
\end{equation}

\kz{the worry about this double-layer transformation is that, $\pi_\theta$, might not be a perfect predictor for the optimal $a$ at  $(s,g)$, which might introduce additional error.}
This essentially says that you train the residual policy to transform optimal actions for some goal $g_i$ in the training set to optimal actions for other goals in the training set $g_j$, assuming time alignment for now. 

Now at test time, when a new goal $g_{\text{test}}$ is drawn from a test distribution $p_{\text{test}}(g)$, such that $g_{\text{test}} - g$ for some $g$ in the training set is in the distribution of $p_{\text{train}}(\delta(g))$ of goal differences that were seen at training time, then we'd expect that the residual function can be applied to transform the actions from the policy applied to goal $g$ in the training set to appropriately get actions to reach $g_{\text{test}}$. 

Specifically, at test time at a particular state $s$ a suitable $g$ is chosen from the training set\kz{how do we choose this $g$ when only seeing $g_{\text{test}}$?}, the ``in-distribution" action is computed using $a = \pi(a|s, g)$ and then this action is transformed via the residual policy $g_\phi(a'|a, g_{\text{test}} - g)$. 

The challenge here is really that while both $a$ and $g_{\text{test}} - g$ have been seen before, they may not have been seen in combination, making the joint $(a, g_{\text{test}} - g)$ potentially out of distribution. So the function $g_\phi$ has to generalize particularly well to new combinations of $(a, g_{\text{test}} - g)$. But the win might be that nothing is out of support (?). This would need some careful thought. \kz{I am not sure if this true. consider the case that ``goal-difference'' seen at testing time can still be out of the support of the ``goal-diff'' seen at training time?}

A couple of things might make this a bit easier to logically reason through. Firstly, instead of having the residual policy $g_\phi(a'|a, g_{\text{test}} - g)$ be a monolithic policy that takes in both $a$ and $g_{\text{test}} - g$, we can break it up into two functions: 

\begin{align}
    & \psi = g_\phi(g_{\text{test}} - g) \\
    & a' = h_\psi(a), \quad a \sim \pi_\theta(a \mid s, g))
\end{align}

This makes the distribution shift a bit more clear, it says that the residual policy produces the parameters $\psi$ for a transformation function $h_\psi$. The inputs to $g_\phi$ are now fully in distribution\kz{I am a bit unsure about this}, but $h_\psi$ for a particular $\psi$ may receive actions to transform $a$ that are unseen and ``out-of-distribution"\kz{I guess this argument also relies on a good generalization of $g_\phi$?}. The solution to this empirically has been to use simple parametrizations (like linear, polynomial or small/simple neural nets) for $h_\psi$ which allows it to extrapolate pretty well. 

However, I think with a bit more care about which goals to compare during the training phase via the sampling distribution $p(i, j)$, I think we can actually avoid this extrapolation issue. The point would be that the distribution of actions $p(a)$ that a particular $h_\psi$ is trained on is critically dependent on the distribution of $p(i, j)$ during training time and carefully modifying this may ensure that new $a$ to transform will still be in distribution. (TODO: Need to make this more concrete). 


A scheme like this seems to be pretty effective in 2d environments


\begin{figure}[!h]
    \centering
    \includegraphics[width=0.35\linewidth]{figs/extrapol.png}
    \caption{Performance on out of distribution points with residual policy}
    \label{fig:ood_res}
\end{figure}


\subsection{}
\newcommand{\pihat}{\hat{\pi}}
\newcommand{\psiin}{\psi_{\mathrm{in}}}
\newcommand{\psiout}{\psi_{\mathrm{out}}}
\newcommand{\dg}{d_{\mathrm{g}}}
\newcommand{\dout}{d_{\mathrm{out}}}

$g = \psi(g)$

$\phi_{\theta}:\cX \to \R^{\dout \times \dg}$, $h_{\psi}: \cG \to \tilde{\cG}$, the policy factors as, $\psi = (\psiin,\psiout)$
\begin{align*}
    \pihat_{\psi}(s,g) = q_{\psiout}(\phi_{\psiin}(s) \cdot g)
\end{align*}
Suppose that, given $\pi_{\theta}$,
\begin{align*}
    \exists \psi_{\star} : \pihat_{\psi_\star} \approx \pi_{\theta}
\end{align*}
\begin{align*}
    \pi_{\theta}(g',s) =  q_{\psiout}(g' \cdot \phi_{\psiin}(s) ) = q_{\psiout}((g' - g) \cdot \phi_{\psiin}(s) + g\phi_{\psiin}(s) ) .
\end{align*}

\begin{align}
    & \psi = f_\phi(g_{\text{test}} - g) \\
    & a' = h_\psi(a,s) \text{s.t} a = \pi_\theta( s, g)
\end{align}

\newcommand{\Rade}{\mathscr{R}}
\begin{align}
    & \psi(g,g') = f_\phi(g' - g) \\
    & \pi_{\theta}(s,g') = h_{\psi(g,g')}(\pi_{\theta}(s,g),s).
\end{align}

There are cases where you can't represent $\pi_{\theta}(s,g)$ as a spline, but, when you have $a = \pi_{\theta}(s,g)$, then you can represent $\pi_{\theta}(s,g')$ as a spline in $s$ \emph{and in } $a$.

Suppose loss
\begin{align*}
    V_{T} = \sum_{t=1}^T \ell_t(\phi \mid s,g,g',a), \text{where}\,\,
    \ell_t(\phi \mid s,g,g',a) =  \|h_{\psi(g,g')}(a,s) - a\|^2
\end{align*}
Now
\begin{align*}
    \|h_{\psi(g,g')}(a,s) - a\|^2 = \| (\sum_{i=1}^k \Phi_i(a,s) f_{\phi,i}(g' - g)) - a \| = \| \Phi(a,s) \cdot f_{\phi}(g' - g)) - a \|^2
\end{align*}
\begin{align*}
     f_{\phi}(g' - g)  \mapsto \ell_t(\phi \mid s,g,g',a) = \| \Phi(a,s) \cdot f_{\phi}(g' - g)) - a \|^2 \text{ is convex}. 
\end{align*}

$\max_{s,a}\|\Phi(a,s) \|_{op} \cdot \Rade_T(\cG) $

Retrain $\phi_t$ at each time $t$ according to an algorithm you would never run, then 
\begin{align*}
    \sum_{t=1}^T \ell_t(\phi_t \mid s,g,g',a)  - \inf_{\phi} \sum_{t=1}^T \ell_t(\phi \mid s,g,g',a) \le \max_{s,a}\|\Phi(a,s) \|_{op} \cdot \Rade_T(\cG).
\end{align*}

Advantage: preserves convexity in $g_\psi$.

\begin{align*}
    \ell_t(\phi \mid s,g,g',a) &= \| \Phi(a,s) \cdot f_{\phi}(g' - g)) - a \|^2 \\
    &= \langle f_{\phi}(g' - g)), \Phi(a,s)^\top \Phi(a,s)  f_{\phi}(g' - g)) \\
    &:= \ell_t(\phi; s,a \mid g,g'). 
\end{align*}

\begin{align}
    \min_{\phi} \max_{s,a: \exists g: a = \pi(s,g)}  \ell_t(\phi; s,a \mid g,g'). 
\end{align}

\begin{align}
    \mathrm{span}(\Phi(s,a) : (s,a,g) : g \in \cG_{\mathrm{train}}) \supset  \mathrm{span}(\Phi(s,a) : (s,a,g) : g \in \cG_{\mathrm{test}})
\end{align}

Featurization of actions that you've taken in the test have to be in the span of actions you've taken. Write out the pseudocode for the whole algorithm. 

==> body/tasks.tex <==
\section{Task Ideas}

\subsection{Tasks for Matrix Completion}
Here are some task ideas for the purely matrix completion. The idea is that we are going to assume that elements are generally seen with high coverage in certain pairs of combinations but not in the bottom right corner of the matrix. The criteria is that the transformation function should be approximately low rank, but the behavior does really have to be different across different combinations, not simply invariant. 

\begin{enumerate}
	\item Different objects doing different tasks. One side of the axis is different objects like cups, mugs, bottles, etc, and the other axis is tasks like pushing, picking, rotating, etc. The idea is that each of these will behave differently but combinatorially it makes a lot more sense to do things through our low rank approximation. 
	\item Multi-task, multi-robot settings. We've seen some examples of robot set A doing task set A and task set B \emph{and} robot set B doing task set A, but not task set B. We'd like to be able to then have robot set B also be able to perform task set B, leveraging the low rank structure of the problem. 
	\item Considering more generally scenarios with varying dynamics and varying tasks. We could consider problems with varying physics parameters and goal locations, and generalize to situations where we have novel physics/goal parameterizations. 
	\item Consider situations where we are manipulating different sized shoes and we do multiple different tasks with them - put them away, pick them up, tie the laces, push them, etc. We want to generalize to new shoe/task combinations. 
	\item We discussed an example with books and bottles. Books and bottles have pretty different styles of being grasped but once they are grasped then we can behave fairly similarly with them. 
	\item We can more generally consider scenarios where we have functional grasping. Different objects have different types of functional grasps and these can be composed to get new combinations.
	\item We can also think about objects which have perception differences, but different tasks, train one thing as a conv embeddng and then add a policy at the end to do prediction.
\end{enumerate}

I think these types of tasks are fairly easy to construct, especially from the literature on GNNs and so on. It also allows us to get away from RL and just do 1 step prediction which will be a lot more effective. 

\subsection{Tasks for Transduction + Matrix Completion}

Here are some task ideas for transduction together with matrix completion. The main ideas that are important here are that we get external validity with the difference operator and the transformation is not just trivially encoded: 

\begin{enumerate}
	\item Obstacles: Consider predicting paths/waypoints/actions for tasks with varying obstacle positions. The behavior change is not quite linear/simple.
	\item Varying weight of an object: Considering predicting how to push an object when it has varying weight distributions. For instance a dumbell with the different sides varying a lot in weight. The difference in weights might be externally valid, but the transformation may not be trivial. 
	\item Car driving to different locations: Even if the difference  in target locations is linear, the transformation on actions is non-linear and potentially low rank. 
	\item Reaching/pushing to different locations but with joint space control. While the trasnsformations in end effector space are trivial, the transformations in joint space are non trivial, although low rank. 
	\item Pushing around multiple objects to different locations but having the objects themselves be in new positions. The differences in position are likely in distribnution even if the object positions themselves are not. 
	\item Manipulating (maybe grasping) objects of different shapes. The comparator between shapes has to be defined as some voxel grid difference but the transduction could work as long as the shape comparator is sensible. 
	\item Grasping an object in various different places and being robust to the changes in behavior depending on the grasp location. For instance, grasping a bottle at the top versus the middle versus the bottom would give different, non-linearly connected behavior. 
	\item Stacking plates with different size and weight with force based control. The size and weight might be externally valid but their connection to change in force/action is non linear. 
	\item Mazes with varying wall positions/configurations and transforming behavior transductively between them. 
	\item Manipulating objects on different surfaces with known friction/surface parameters but with force based control/joint space control.
\end{enumerate}

==> body/theory_simple.tex <==
%!TEX root = ../main_simple.tex

\newcommand{\Iobs}{\cI_{\mathrm{obs}}}


\section{Theoretical Overview}
We present a stylized version of our results. Our aim is to learn a function $\hst(x,y): \xspac \times \yspace \to \R$, using the assumption that it  has a low-rank  structure. Specifically, we assume that there exist embeddings into a  potentially infinite-dimensional Hilbert space $\fst:\xspac \to \hilspace$ and $\gst: \yspace \to \hilspace$ for which all triples are of the form
\begin{align}
(x,y,z) = (x,y,\hst(x,y)), \quad \hst(x,y) \equiv \langle \fst(x), \gst(y) \rangle. \label{eq:low_rank}
\end{align}
Our goal is to learn the function $\hst$; \textbf{We omit noise for simplicity, though our analysis extends to the case with sub-Gaussian noise as well.}  

 Specifically, we study how \Cref{eq:low_rank} facilitates a   form of out-of-support extrapolation, when the embeddings $\fst,\gst$ satisfy certain regularity guarantees. Suppose that our input spaces decompose as $\xspac = \xspac_1 \cup \xspac_2$, $\yspace = \yspace_1 \cup \yspace_2$. Our goal is to learn $\hst$ on $\xspac_2 \times \yspace_2$ given access to samples covering $\xspac_i\times \yspace_j$ for pairs $(i,j) \in \{(1,1),(1,2),(2,1)\} := \Iobs$ (we call these the \emph{observed blocks}) . 

\begin{figure}[ht]
 {\centering
 \hspace{-10pt}   
 \includegraphics[width=0.25\linewidth]{figs/simple_fig_1_a.png}
 \quad  
 \hspace{-9pt} 
 \includegraphics[width=0.444\linewidth]{figs/simple_fig_1_b.png}    
 \quad~~    
 \includegraphics[width=0.25\linewidth]{figs/simple_fig_1_c.png}\vspace{0pt}}\\ 
 \vspace{-10pt} 
 \hspace{58pt}(a) \hspace{150pt} (b)  \hspace{158pt} (c) \\  
\caption{\emph{(a)}. Illustration of $\bM^*\in\R^{M\times N}$.  \emph{(b)}. The embeddings $\bA^\star$ and  $\bB^\star$, of dimension $\nu=\min\{M,N\}$. 
% ,  and similarly  $A^{\btheta},B^{\btheta}$ analogously.  Enforcing the embedding to have dimension $k$ is equivalent to enforcing $M^\star$ and $M^{\btheta}$ have rank $\le k$. 
\emph{(c)}. Illustration of the sampling and missing data patterns. 
% Consider a setting, where, (after a permutation), the train indices are uniform on 
}\label{fig:matrix_illustration}
\end{figure} 

Throughout, we give examples motivated by matrix completion. We denote the $(a,b)$-th entry of a matrix $\bM$ by $\bM_{[ab]}$, and use $\bM_{i,j}$ to denote block matrices (the block decomposition will be clear from context). The following example is helpful: 

\begin{example}\label{exmp:finite} $\xspac= \{x_1,\dots,x_N\}$ and $\yspace = \{y_1,\dots,y_M\}$, where  $N$ and $M$ are very large. Then, we can view $\hst(x,y)$ as defining  a matrix $\bstM \in \R^{N \times M}$ via $\bstM_{[ab]} = \hst(x_a,y_b)$ (see Figure \ref{fig:matrix_illustration} (a)). Without loss of generality, $\fst,\gst$ map to dimension $\nu = \min\{N,M\}$. Then, by setting $\bstA_{[ac]} = \fst_{[c]}(x_a)$ and $\bstB_{[bd]} = \gst_{[d]}(y_b)$, we recover a factorization $\bstM = \bstA(\bstB)^\top$ (see Figure \ref{fig:matrix_illustration} (b)).  
% \mscomment{See figure 1-b}




For $N_1 \le N$,  let $\xspac_1 = \{x_a: a \in [N_1]\}$, and let $\xspac_2 = \xspac \setminus \xspac_1$ denote the remaining indices. Similarly, for $M_1 \le M$, let $\yspace_1 = \{y_b: b \in [M_1]\}$ and $\yspace_2 = \yspace \setminus \yspace_1$. Then spaces $\xspac_i \times \yspace_j$ denote the covariates associated to the $(i,j)$-block of $\bstM$, and our goal is then to ``complete'' the $(2,2)$ block from samples in the other blocks (see Figure \ref{fig:matrix_illustration} (c)). We shall revisit this example frequently, and set $N_2 = N - N_1$ and $M_2 = M - M_1$.  
\end{example}

\newcommand{\xsp}{\xspac}
\newcommand{\ysp}{\yspace}
\subsection{Distributional Setting}

We aim for results for the cases where the spaces  $\xsp,\ysp$ are very large or perhaps infinite. Therefore, we need distributional and function-approximation conditions.  Specifically, we assume that there exist distributions $\cD_{\xsp,i}$ supported on $\xsp_i$ and $\cD_{\ysp,j}$ on $\ysp_j$ for $i,j \in \{1,2\}$. As shorthand, we define the product distributions $\disij := \cD_{\xsp,i} \otimes \cD_{\ysp,j}$. For an arbitrary distribution $\cD$ on $\xspac \times \yspace$, we introduce the $\cL_2$-risk
\begin{align*}
\Risk(f,g;\cD) := \Exp_{(x,y) \sim \cD}[(\langle f(x),g(y) \rangle - \hst(x,y))^2].
\end{align*}
\paragraph{A. Test Distribution \& Extrapolation.} 
Our aim is to train on a certain training distribution $\Dtrain$ so as to have low-risk on the unobserved, $(2,2)$-block. Specifically, we aim to ensure
\begin{align}
\Risk(f,g;\cD_{2\otimes 2}) = \Exp_{x \sim \cdxtwo}\Exp_{y \sim \cdytwo}[(\langle f(x),g(y) \rangle - \hst(x,y))^2]\le \epsilon_{\mathrm{targ}}^2. \label{eq:extrapolation}
\end{align}
Because we only require acccess to samples from $\disij$ for $(i,j) \ne (2,2)$, we refer to attaining \Cref{eq:extrapolation} as \emph{extrapolation}. This is in distinction to \emph{generalization}, which regards generalizing from a training distribution to test samples from the \emph{same} distribution. 

\begin{example}[Uniform Test Distribution]\label{exm:finite_test} Returning to \Cref{exmp:finite}, let $\cdxi = \Unif(\cX_i)$ and $\cdyj = \Unif(\cY_j)$ be the uniform distributions on their supports. Then, the goal is to learn embeddings $\fhat,\ghat$ whose inner products $\langle \fhat,\ghat \rangle$ is close to to $\hst(x,y)$ on entries  $(x,y)$ drawn uniformly from $\xsp_2 \times \ysp_2$.   This admits an interpretation as Frobenius norm recovery. Namely, recall the identification $\bstM_{[ab]} = \hst(x_a,y_b)$, and define $\bhatM_{[ab]} := \langle \fhat(x_a),\ghat(y_b) \rangle$. Letting $\bstM_{2,2}$ and $\bhatM_{2,2}$ denote the bottom block corresponding to  indices in $\xsp_2 \times \ysp_2$, i.e., 
\begin{align*}
\Risk(\fhat,\ghat;\cD_{2\otimes 2}) = \frac{1}{N_2M_2}\fronorm{\bstM_{2,2}-\bhatM_{2,2}}^2.
\end{align*}
\end{example}
\begin{example}[Non-Uniform Test] Again, consider the discrete setting of \Cref{exmp:finite}, but instead suppose the distributions are \emph{non-uniform}. Let $\bp^{(i)} \in \R^{N_i}$  denote the probability vector  for which $\Pr_{x' \sim \cdxone}[x' = x] = \bp^{(1)}_x$, and let $\bp^{(2)}$ be such that $\Pr_{x' \sim \cdxtwo}[x' = N_1 + x] = \bp^{(2)}_{x}$\kz{made the changes here so that the Diag below matches the dimension.}.  Define probability vectors $\bq^{(1)},\bq^{(2)}$ analogously for the $y$-features. Then, 
\begin{align*}
\Risk(f,g;\cD_{2\otimes 2}) = \fronorm{\Diag(\bp^{(2)})^{\frac{1}{2}}(\bstM_{2,2}-\bhatM_{2,2})\Diag(\bq^{(2)})^{\frac{1}{2}}}^2,
\end{align*}
that is, the $\cL_2$ risk corresponds to a weighted Frobenius norm. 
\end{example}

\paragraph{B. Structure of Training Distribution.} We now specify the form of our training distribution: 

\begin{assumption}\label{asm:dtest} We have access to samples from a  \emph{training} distribution $(X,Y,Z) \sim \Dtrain$ where $Z= \hst(X,Y)$ with probability one, and which covers $\disij$, for $(i,j) \in \Iobs = \{(1,1),(1,2),(2,1)\}$ in the following sense: letting $\rmd$ denote the Radon-Nikodym derivative (or density), we assume there is a constant $c > 0$ such that
\begin{align*}
 \frac{\rmd \Dtrain(x,y)}{\sum_{(i,j)\in \Iobs} \rmd\disij(x,y)}  = \frac{\rmd \Dtrain(x,y)}{\sum_{(i,j)\in \Iobs} \rmd\cdxi(x)\rmd\cdyj(y)} \ge 1/c.
\end{align*}
\end{assumption}
\begin{example}\label{exm:finite_train} Returning to \Cref{exmp:finite}, for block indices $i,j \in \{1,2\}$, let $\cdxi = \Unif(\cX_i)$ and $\cdyj = \Unif(\cY_j)$ be the uniform distributions on their supports. Then, the mixture distribution, which selects an $(i,j)$ uniformly from the observed blocks $\Iobs$, and samples $x \sim \Unif(\cX_i)$ and $y \sim \Unif(\cX_j)$ satisfies \Cref{asm:dtest} with $ c= 1/3$. In fact, \Cref{asm:dtest} holds for the same construction with arbitrary $\cdxi$ and $\cdyj$, but $(i,j)$ chosen uniformly on $\Iobs$, with $c = 1/3$. 

Another valid construction is as follows. Suppose that the cardinalities $N = |\xsp|$ and $M = |\ysp|$, as well as $N_1 = |\xsp_1|$ and $M_1 = |\ysp_1|$ satisfy $N \ge \alpha N_1$ and $M \ge \beta M_1$. Let $\Dtrain$ be the uniform distribution on all indices in the observed blocks, $\bigcup_{(i,j) \in \Iobs} \xsp_i \times \ysp_j$.  Then, \Cref{asm:dtest} holds with $c = \alpha\beta/3$.
\end{example}
\newcommand{\epshat}{\hat{\epsilon}}
\newcommand{\trainorac}{\bmsf{train}}
\newcommand{\distorac}{\bmsf{distill}}
\newcommand{\rdistill}{\cR_{\mathrm{distil}}}
\newcommand{\epsdistill}{\eps_{\mathrm{distil}}}



\paragraph{C. Covariance Structure.} Suppose there is a constant $B > 0$ for which $$\Big\{\sup_{x}\|\fst(x)\|_{\hilspace},~\sup_{y}\|\gst(y)\|_{\hilspace}\Big\} \le B.$$ 
This means that $\Exp_{x \sim \cdxone}[\fst(x)\fst(x)^\adj]$ and $\Exp_{y \sim \cdyone}[\gst(y)\gst(y)^\adj] $ are trace-class operators\kz{shall we explain this argument a bit? Also, it seems a bit unclear what are these mappings map from, and to.}, and we can reparameterize our representation (by change of bases) so as to ensure the embeddings are \emph{balanced}, defining a common trace-class covariance  $\Sigst: \hilspace \to \hilspace$\kz{sorry I might be missed it, and is a bit confused about this notation: $\fst(x),\gst(y)$ lie in $\cH$, right? why $\Sigst$ maps $\cH$ to $\cH$?}  
% should it be something like $\cH\times \cH^\star$ to $\cH\otimes\cH^\star$?}:   
\begin{align*}
\Sigst := \Exp_{x \sim \cdxone}[\fst(x)\fst(x)^\adj] = \Exp_{y \sim \cdyone}[\gst(y)\gst(y)^\adj ]. 
\end{align*}
We let $\projop_k$ denote the projection onto the top $k$-eigenvectors of $\Sigst$. We define the optimal projections of $\fst,\gst$ as
\begin{align*}
\fstk := \projop_k \fst, \quad \gstk := \projop_k \gst.
\end{align*}
\paragraph{D. Function Approximation} Because the embeddings are potentially infinite dimensional, we need to constrain their capacity. For simplicity, we state the most succinct  version of our function-approximation guarantee: realizability of $\fstk,\gstk$ and finite function classes. The following  assumption can be weakened considerably.
\begin{assumption}[Function Approximation]
We assume that there exist,  for each $k \in \N$, finite function classes  $\Fclass_k,\Gclass_k$ with $\capac_k := \log(|\Fclass_k|\cdot|\Gclass_k|)$ for which $\fstk \in \Fclass_k$ and $\gstk \in \Gclass_k$. 
\end{assumption}

\begin{figure}[ht]
 \centering
%  \hspace{-10pt}   
 \includegraphics[width=0.8\linewidth]{figs/simple_fig_2.png}\\  
%  \\  v
% %  \vspace{-10pt} 
%  \hspace{58pt}(a) \hspace{150pt} (b)  \hspace{158pt} (c) \\  
\caption{Illustration of the Relative Covariance Assumption for $\bA^*$, similarly for $\bB^*$.  
}\label{fig:rel_cov_illustration}
\end{figure} 


\paragraph{E. Relative Covariance Assumption.} Even with the above assumptions, it is not in general possible to ensure extrapolation; this can be seen by noting that rank-$1$ matrices of the form
\begin{align*}
\bstM = \begin{bmatrix} 0 & 0 \\ 0 & ?\end{bmatrix} \in \R^{2 \times 2}
\end{align*}
are underdetermined. This pathology is avoided under the following condition:
\newcommand{\sfv}{\bmsf{v}}
\begin{assumption}[Relative Covariance]
We assume that there exists a constant $\kapcov$ such that, for any $\sfv \in \hilspace$ with $\|\sfv\|_{\hilspace} = 1$,
\begin{align*}
\Exp_{x\sim \cdxtwo}\langle \sfv,\fst(x)\rangle^2 \le \kapcov\Exp_{x\sim \cdxone}\langle \sfv,\fst(x)\rangle^2, \quad \Exp_{y\sim \cdytwo}\langle \sfv,\gst(x)\rangle^2 \le \kapcov\Exp_{y\sim \cdyone}\langle \sfv,\gst(x)\rangle^2.
\end{align*}
\end{assumption} 
For the matrix setting of \Cref{exmp:finite} with uniform sampling as in \Cref{exm:finite_train}, this means that the partition under the natural partition of the factors $\bstA,\bstB$ into blocks, that $(\bstA_2)^\top \bstA_2 \preceq   \kapcov (\bstA_1)^\top \bstA_1$ holds, and similarly for $\bstB$. See Figure \ref{fig:rel_cov_illustration} for an illustration.  
% \mscomment{figure} 
\kz{should  we need some justification/intuition for this assumption (or its necessity)? e.g., can we say that it means the ``power'' contained in the (2,2) block 
has to be dominated by that of other blocks? or any other related assumptions in the literature that we might cite?} 
% \newcommand{\gtil}{\tilde{g}}
\newcommand{\Dsvd}{\cD_{\mathrm{dis}}}
\newcommand{\kapdis}{\kappa_{\mathrm{dis}}}
\subsection{Algorithm}
Now we state our algorithm in a stylized setting where empirical risk minimization is assumed to be possible. We use a common sample size $N$ for all procedures. Lastly, we assume \emph{unsupervised } access to samples from a distribution which is a constant multiplicative approximation to $\disone$:
\begin{assumption}[Distillation Oracle] We have access to unlabeled samples   $(X_i,Y_i) \sim \Dsvd$ distillation distribution $\Dsvd$ which satisfy, for some constant $\kapdis \ge 1$, 
\begin{align*}
1/\kapdis \le \frac{\rmd \Dsvd(x,y)}{\rmd\disone(x,y)}  = \frac{\rmd \Dsvd(x,y)}{ \rmd\cdxone(x)\rmd\cdyone(y)} \le \kapdis.
\end{align*}
\end{assumption}
\newcommand{\fred}{f_{\mathrm{red}}}
\newcommand{\gred}{g_{\mathrm{red}}}

Our algorithm consists of four steps. First, we train an overparametrized embeddings $\ftil,\gtil$ on $N$ samples from $\Dtrain$ with embedding dimension $k_0$. Then, we use $N$ unlabeled samples  for $\Dsvd$ to compute a balanced, rank-$k$ approximations $\fred$ and $\gred$. Finally, we train on a combination of samples from $\Dtrain$ and $\Dsvd$ to find a final classifier which has low overall risk, and which is close to the $\fred,\gred$ on samples from $\Dsvd$. We summarize the process in \Cref{alg:main_alg}.  \kz{shall we include a bit more explanation/context why we need this double-training process? what is the intuition/necessity of  distillation? etc.}

 \begin{algorithm}[!t]
    \begin{algorithmic}[1]
    \State{}\textbf{Input: } Sample size $N$; over-parameterized rank $p$, underparametrized cutoff $r_0$, parameter $\sigma_0$, 
    regularization $\mu,\lambda > 0$.
    \State{}\textbf{Overparametrized training.} Sample $N$ \emph{labeled} triples $\{(X_i,Y_i,Z_i)\}_{i=1}^N \sim \Dtrain$, and set
    \begin{align*}
    (\ftil,\tilde g) \in \argmin_{(f,g) \in \Fclass_{p}\times \Gclass_{p}} \sum_{i=1}^N (\langle f(X_i),g(Y_i)\rangle - Z_i)^2. 
    \end{align*}
    \State{}\textbf{Covariance Estimation. }  Sample $N$ \emph{unlabeled} examples $\{(X_i,Y_i)\}_{i=N+1}^{2N} \sim \Dsvd$, and define the regularized covariance matrices
    \begin{align*}
    \hat{\bSigma}_{\ftil} := \frac{1}{n}\sum_{i=1}^n\ftil(X_i)\ftil(X_i)^\top, \quad \hat{\bSigma}_{\gtil} := \frac{1}{n}\sum_{i=1}^n\gtil(X_i)\gtil(X_i)^\top
    \end{align*}
    \State{}\textbf{Dimension reduction.} $(r,\bQ_r) \gets \mathsf{BalancedProjection}(\hat{\bSigma}_{\ftil} +  \mu \eye_p, \hat{\bSigma}_{\gtil} +  \mu \eye_p,r_0,\sigma_0)$.
    \State{}\textbf{Distillation. }  Sample $N$ \emph{unlabeled} examples $\{(X_j,Y_j)\}_{i=2N+1}^{3N} \sim \Dsvd$ and $N$ \emph{labeled} triples $\{(X_i,Y_i,Z_i)\}_{i=3N+1}^{4N} \sim \Dtrain$, and select
    \begin{align*}
    (\fhat,\ghat) \in \argmin_{(f,g) \in \Fclass_r\times\Gclass_r}\hat{\cR}_{\mathrm{sup}}(f,g) + \lambda\hat{\cR}_{\mathrm{dis}}(f,g\mid \ftil,\gtil,\bQ_r),
    \end{align*}
    where we define the distillation and supervised empirical risks as
    \begin{align*}
     \hat{\cR}_{\mathrm{dis}}(f,g\mid\ftil,\gtil,\bQ_r) &:= \sum_{j=2N+1}^{3N}(\langle f(X_j),g(Y_j)\rangle - \langle \ftil(X_j),\bQ_r\cdot\gtil(Y_j)\rangle^2\\
    \hat{\cR}_{\mathrm{sup}}(f,g) &:= \sum_{i=3N+1}^{4N} (\langle f(X_i),g(Y_i)\rangle - Z_i)^2.
    \end{align*}
    \end{algorithmic}
      \caption{Two-Step Completion}
      \label{alg:main_alg}
    \end{algorithm}



    \begin{algorithm}[!t]
    \begin{algorithmic}[1]
    \State{}\textbf{Input: } $\bX,\bY \succ 0$, $r_0 \in \N$, $\sigma_0$. 
    \State{} Compute $\bW := \bX^{\half}(\bX^{\half}\bY \bX^{\half})^{-\half}\bX^{\half}$. 
    \State{} Compute $\bSigma := \bW^{\half} \bY \bW^{\half}$ and
    \begin{align*}
    r \gets  \max\left\{r \in [r_0]: \sigma_r(\bSigma) \ge \sigma_0, \,\sigma_r(\bSigma) - \sigma_{r+1}(\bSigma) \ge \frac{\sigma_r(\bSigma)}{r_0}\right\}
    \end{align*}
    \State{} Let $\bP_r$ denote the projection onto the top $r$ eigenvectors of $\bSigma$.
    \State{} Return $(r,\bQ_r)$, where $\bQ_r \gets \bW^{-\half}\bP_r \bW^{\half}$.
    \end{algorithmic}
      \caption{$\mathsf{BalancedProjection}(\bSigma_{1}, \bSigma_{2}, r_0, \sigma_0)$}
      \label{alg:main_alg}
    \end{algorithm}

\subsection{Guarantees}
We now state an informal version of our  guarantees. The following theorem  illustrates the behavior of \Cref{alg:main_alg} when $\Sigst$ has slow polynomial decay, that is, its  $n$-th eigenvalue decays as $n^{-(1+\gamma)}$ for some $\gamma$  possibly close to $0$. One can derive sharper guarantees in a benign exponential decay setting. 
\begin{theorem}[Informal]\label{thm:main_informal} Fix a failure probability $\delta \in (0,1)$ and target accuracy $\epsilon$. Suppose that for some $\gamma > 0$, the spectrum of $\Sigst$ decays as $\lambda_n(\Sigst) \le Cn^{-(1+\gamma)}$ (polynomial decay) for some constant $C>0$. Then, for a given $\epsilon$, there exist rank choices $k \le k_0 \le \epsilon^{-\BigOh{1/\gamma}}$, such that the output of \Cref{alg:main_alg} with suitable regularization parameter  $\lambda$ satisfies
\begin{align*}
\Pr[\Risk(\fhat,\ghat;\distwo) \ge \epsilon] \le \delta.
\end{align*}
provided that the sample size $N \ge (\log(1/\delta)\capac_{k'})^{\BigOh{1}} \cdot \epsilon^{-\BigOh{1/\gamma}}$  for some constant  $C_{k'}$ and any $\epsilon<1$. 
\end{theorem}
\newcommand{\unseen}{\textbf{?}}

\subsection{Comparison to Existing Work} This subsection  provides a brief summary of related work, to the best of our knowledge.  
% sketches related work, as we understand it. 
To facilitate  comparison, we consider a ground-truth matrix $\bstM \in \R^{M \times N}$ as the matrix to be completed. $\bM \in \R^{M \times N}$ is a noisy realization of $\bstM$ with $\Exp[\bM] = \bstM$, and we assume that we are given observed matrix $\btilM \in (\R \cup \{\unseen\})^{M \times N}$, where `$\unseen$' denotes an unseen entry, such that $\btilM_{[ab]}= \bM_{[ab]}$ unless $\btilM_{[ab]} =\,\unseen$. We let $\bD \in \{0,1\}^{M \times N}$ denote the masking matrix of $\btilM$: $\bD_{[ab]} = \I\{\btilM_{[ab]} \ne \,\unseen\}$.   

\paragraph{Missing-completely-at-random (MAR) matrix completion.} In the MAR setting, it is assumed that the entries of $\bD$ are i.i.d. Bernoulli random variables with positive probability $p > 0$ and independent of $\bM$; some existing works include  \cite{candes2010power,recht2011simpler,hastie2015matrix,mazumder2010spectral,koltchinskii2011nuclear}. More recent works study settings where $\bstM_{[ab]}$ is generated by bivariate function $\hst(x_a,y_b) = \langle \fst(x_a),\gst(y_b)\rangle$ of features $x_a,y_b$; in  \citep{xu2018rates}, this encodes graphon structure, whereas in \cite{song2016blind,li2019nearest}, $\hst(x,y)$ is a globally Lipschitz function, which admits learning via matrix completion by considering linearizing expansions. \cite{yu2021nonparametric} considers an extension to the ``one-sided'' covariate setting that is more  challenging, where only the first argument of $\hst$ is observed. A ``one-bit'' sensing model has also been studied in  \cite{davenport20141}, and refined under a latent variable model for features $x_a,y_b$ \citep{borgs2017thy}. All aforementioned works consider the MAR setting. 

\paragraph{Missing at random.} In the missing-at-random setting, it is assumed that there exists a set of observed covariates $\cO$ such that $\bM \perp \bD \mid \cO$\kz{for this notation, do we mean $(\bM \perp \bD) \mid \cO$ or $\bM \perp (\bD \mid \cO)$?}, and that $\bD_{[ab]} \mid \cO$ are independent Bernoulli random-variables with possibly different probabilities $p_{ab}$ uniformly bounded below. See e.g. \cite{schnabel2016recommendations,wang2018modeling,liang2016modeling}. 


\paragraph{Missing not at random (MNAR).} 
% \mscomment{Define}. 
Many works consider generative models, relating missingness of entries to either ground-truth or realized-values of the matrix via logistic expressions \citep{sportisse2020imputation,yang2021tenips}. Guarantees obtained from this strategy typically depend on a lower bound on the minimal probability that an entry is revealed \citep{ma2019missing}, dependence on which is also incurred in an alternative approach due to \cite{bhattacharya2022matrix}. Note that in our setting, we allow the entries of $\bstM_{2,2}$ to be \emph{entirely} omitted from $\btilM_{2,2}$, so these guarantees are vacuous here. Another approach due to \cite{foucart2020weighted} studies reconstruction from MNAR data under weighting matrices that are suitably calibrated to the pattern of missing entries. Again, in our setting, these results become vacuous. 

Two more recent works establish recovery for entries which are indeed missing with  probability one. \cite{shah2020sample} considers almost precisely our  setting, where, motivated by reinforcement learning, one attempts to recover $\bstM_{2,2}$ by observing the other blocks $\bstM_{1,2},\bstM_{2,1},\bstM_{2,2}$. However, their results require that either (a) $\bstM$ is exactly low rank, or (b) that $\bstM$ is approximately low rank, but that the error between $\bstM$ and its rank-$r$ SVD is very small entry-wise. This  precludes the much more gradual polynomial decay allowed by \Cref{thm:main_informal}. A second work, \cite{agarwal2021causal}, considers far more general patterns of missing entries than we do in this work. However, this comes at the cost of requiring even stronger assumptions on the spectrum \citep[Assumption 6]{agarwal2021causal}, which again preclude approximately low-rank matrices with spectral decay. 

\paragraph{Claimed Novelty.} To our knowledge, this is the first work which recovers an {\it approximately}  low-rank matrix (i.e. a matrix with at least $\lambda_n \le n^{1+\alpha}$ \kz{$\lambda_n \le 1/n^{1+\alpha}$?} spectral decay for $\alpha > 0$) \kz{could we give some justification/or maybe examples, about the significance of this ``generality'' (especially in practical problems)?} in a truly MNAR setting where some entries are non-observed with probability zero. 

\mscomment{Double Training Algorithm, Analysis Tools, Flexibility in the Sampling } 




==> preamble/reg_macros.tex <==
\newcommand{\lbr}{\lbrace}
\newcommand{\rbr}{\rbrace}

\newcommand{\ac}{{A_c}}
\newcommand{\bc}{{B_c}}
\newcommand{\cc}{{C_c}}
\newcommand{\dc}{{D_c}}

\newcommand{\cparams}{\ac,\bc,\cc,\dc}
\newcommand{\lmiparams}{X,Y,K,L,M,N}

%\newcommand{\transp}{^{\top}}
\newcommand{\invtransp}{^{-\top}}
\newcommand{\inv}{^{-1}}



\newcommand{\params}{\x}
\newcommand{\obj}{F}
\newcommand{\regf}{R}
\newcommand{\ccg}{\Sigma}
\newcommand{\robj}{G}

%\newcommand{\h}{h}
\newcommand{\dt}{\bar{T}}

\newcommand{\simt}{\mathcal{S}}
\newcommand{\shot}{\mathcal{S}_{\textup{hot}}}

\newcommand{\stpt}[1]{\bar{#1}}

\newcommand{\spoint}{\stpt{\params}}

%\newcommand{\xcl}{\mathcal{X}}
%
%\newcommand{\x}{\mathbf{x}}
%\newcommand{\y}{\mathbf{y}}
\newcommand{\bnu}{\boldsymbol{\nu}}
\newcommand{\ytmp}{\bnu}

\newcommand{\dir}{\mathbf{d}}

\newcommand{\xc}{\bar{x}}

\newcommand{\miniheading}[1]{
	{\vspace{0.5em}
		\parindent0pt 
		\textbf{#1} \\
	}
}

\newcommand{\hot}{\textup{h.o.t}}
